Dividable Configuration Performance Learning

Machine/deep learning models have been widely adopted for predicting the configuration performance of software systems. However, a crucial yet unaddressed challenge is how to cater for the sparsity inherited from the configuration landscape: the influence of configuration options (features) and the distribution of data samples are highly sparse. In this paper, we propose a model-agnostic and sparsity-robust framework for predicting configuration performance, dubbed DaL, based on the new paradigm of dividable learning that builds a model via "divide-and-learn". To handle sample sparsity, the samples from the configuration landscape are divided into distant divisions, for each of which we build a sparse local model, e.g., regularized Hierarchical Interaction Neural Network, to deal with the feature sparsity. A newly given configuration would then be assigned to the right model of division for the final prediction. Further, DaL adaptively determines the optimal number of divisions required for a system and sample size without any extra training or profiling. Experiment results from 12 real-world systems and five sets of training data reveal that, compared with the state-of-the-art approaches, DaL performs no worse than the best counterpart on 44 out of 60 cases with up to 1.61x improvement on accuracy; requires fewer samples to reach the same/better accuracy; and producing acceptable training overhead. In particular, the mechanism that adapted the parameter d can reach the optimal value for 76.43% of the individual runs. The result also confirms that the paradigm of dividable learning is more suitable than other similar paradigms such as ensemble learning for predicting configuration performance. Practically, DaL considerably improves different global models when using them as the underlying local models, which further strengthens its flexibility.

==> Figures/Tradeoff.tex <==

% \begin{figure}[!t]
% \centering
% \footnotesize
\begin{subfigure}{.31\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/Apache_tradeoff.jpg}  
  \caption{\textsc{Apache}}
  \label{fig:tradeoff-Apache}
\end{subfigure}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/BDBC_tradeoff.jpg} 
  \caption{\textsc{BDB-C}}
  \label{fig:tradeoff-BDBC}
\end{subfigure}
\begin{subfigure}{.33\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/BDBJ_tradeoff.jpg} 
  \caption{\textsc{BDB-J}}
  \label{fig:tradeoff-BDBJ}
\end{subfigure}

\begin{subfigure}{.31\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/x264_tradeoff.jpg}  
  \caption{\textsc{x264}}
  \label{fig:tradeoff-x264}
\end{subfigure}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/hsmgp_tradeoff.jpg} 
  \caption{\textsc{HSMGP}}
  \label{fig:tradeoff-Hsmgp}
\end{subfigure}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/hipacc_tradeoff.jpg}  
  \caption{\textsc{HIPA$^{cc}$}}
  \label{fig:tradeoff-hipacc}
\end{subfigure}


\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/VP8_tradeoff.jpg} 
  \caption{\textsc{VP8}}
  \label{fig:tradeoff-VP8}
\end{subfigure}
% \hspace{5mm}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/Irzip_tradeoff.jpg} 
  \caption{\textsc{Lrzip}}
  \label{fig:tradeoff-Lrzip}
\end{subfigure}
\hspace{4mm}
\begin{subfigure}{.15\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/legend.png} 
%   \label{fig:legend}
%   \vspace{8mm}
\end{subfigure}

%     \caption{The total Scott-Knott scores for each subject system on both time and MRE. Only the Pareto-optimal models are presented.}
%     \label{fig:tradeoff}
% \end{figure}

==> Figures/response_box_plot.tex <==
\begin{adjustbox}{width=1\textwidth,center}
\begin{subfigure}{.175\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/Apache_AllNumeric_MRE_diff_boxplot.png} 
      \subcaption{\textsc{Apache}}
\end{subfigure}
\begin{subfigure}{.158\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/BDBC_AllNumeric_MRE_diff_boxplot.png} 
  \subcaption{\textsc{BDB-C}}
\end{subfigure}
\begin{subfigure}{.149\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/BDBJ_AllNumeric_MRE_diff_boxplot.png} 
  \subcaption{\textsc{BDB-J}}
\end{subfigure}
\begin{subfigure}{.158\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/kanzi_MRE_diff_boxplot.png} 
 \subcaption{\textsc{kanzi}}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/sqlite_MRE_diff_boxplot.png} 
  \subcaption{\textsc{SQLite}}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/x264_AllNumeric_MRE_diff_boxplot.png} 
  \subcaption{\textsc{x264}}
\end{subfigure}
\end{adjustbox}

\vspace{0.2cm}

\begin{adjustbox}{width=1\textwidth,center}
\begin{subfigure}{.17\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/Dune_AllNumeric_MRE_diff_boxplot.png} 
 \subcaption{\textsc{Dune}}
\end{subfigure}
\begin{subfigure}{.165\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/hipacc_AllNumeric_MRE_diff_boxplot.png} 
  \subcaption{\textsc{HIPA$^{cc}$}}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/hsmgp_AllNumeric_MRE_diff_boxplot.png} 
  \subcaption{\textsc{HSMGP}}
\end{subfigure}
\begin{subfigure}{.158\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/Lrzip_MRE_diff_boxplot.png} 
  \subcaption{\textsc{Lrzip}}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/nginx_MRE_diff_boxplot.png} 
 \subcaption{\textsc{nginx}}
\end{subfigure}
\begin{subfigure}{.165\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/VP8_MRE_diff_boxplot.png} 
 \subcaption{\textsc{VP8}}
\end{subfigure}
\end{adjustbox}

==> Figures/response_sensitivity_to_depth.tex <==
% \begin{figure}[!t]
% \centering
% \footnotesize
\begin{subfigure}{.3\columnwidth}
  \centering
  
    % include first image
\includegraphics[width=\linewidth]{Figures/Apache_AllNumeric_depths.png}  
  \subcaption{\textsc{Apache}}
  \label{fig:depth-Apache}
\end{subfigure}
~%\hspace{-0.1cm}
\begin{subfigure}{.3\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/BDBC_AllNumeric_depths.png} 
  \caption{\textsc{BDB-C}}
  \label{fig:depth-BDBC}
\end{subfigure}
~
\begin{subfigure}{.3\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/BDBJ_AllNumeric_depths.png} 
  \subcaption{\textsc{BDB-J}}
  \label{fig:depth-BDBJ}
\end{subfigure}

\vspace{0.2cm}

\begin{subfigure}{.3\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/kanzi_depths.png}  
  \subcaption{\textsc{kanzi}}
  \label{fig:depth-kanzi}
\end{subfigure}
~
\begin{subfigure}{.3\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/sqlite_depths.png} 
  \subcaption{\textsc{SQLite}}
  \label{fig:depth-sqlite}
\end{subfigure}
~%\hspace{-0.1cm}
\begin{subfigure}{.3\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/x264_AllNumeric_depths.png}  
  \subcaption{\textsc{x264}}
  \label{fig:depth-x264}
\end{subfigure}

\vspace{0.2cm}

\begin{subfigure}{.3\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/Dune_AllNumeric_depths.png} 
  \subcaption{\textsc{Dune}}
  \label{fig:depth-Dune}
\end{subfigure}
~%\hspace{-0.1cm}
\begin{subfigure}{.3\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/hipacc_AllNumeric_depths.png} 
  \subcaption{\textsc{HIPA$^{cc}$}}
  \label{fig:depth-hipacc}
\end{subfigure}
~
\begin{subfigure}{.3\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/hsmgp_AllNumeric_depths.png} 
  \subcaption{\textsc{HSMGP}}
  \label{fig:depth-Hsmgp}
\end{subfigure}

\vspace{0.2cm}

\begin{subfigure}{.3\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/Lrzip_depths.png} 
  \subcaption{\textsc{Lrzip}}
  \label{fig:depth-Lrzip}
\end{subfigure}
~
\begin{subfigure}{.3\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/nginx_depths.png} 
  \subcaption{\textsc{nginx}}
  \label{fig:depth-nginx}
\end{subfigure}
~%\hspace{-0.1cm}
\begin{subfigure}{.3\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/VP8_depths.png} 
  \subcaption{\textsc{VP8}}
  \label{fig:depth-VP8}
\end{subfigure}



==> Tables/RQ1-individual-table.tex <==
% %% The first command in your LaTeX source must be the \documentclass command.
% \documentclass[manuscript]{acmart}
% %% NOTE that a single column version may be required for 
% %% submission and peer review. This can be done by changing
% %% the \doucmentclass[...]{acmart} in this template to 
% %% \documentclass[manuscript,screen]{acmart}
% %% 
% %%
% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}
    


% \newcommand{\Model}{\texttt{DaL}} % name of the model

% \usepackage[ruled, linesnumbered, vlined, commentsnumbered]{algorithm2e}
% \usepackage{xcolor,colortbl}
% \usepackage{multirow}
% \usepackage{subcaption} % for subfigure
% \usepackage{tcolorbox}
% \usepackage{csquotes}
% \usepackage{adjustbox}
% \usepackage{geometry}
% % \usepackage[figuresright]{rotating}
% \geometry{a4paper,left=0cm,right=0cm,top=0cm,bottom=0cm}
% \usepackage{tabularx} % in the preamble
% \newtcolorbox{quotebox}{colback=white!10,boxrule=0.4pt,colframe=black,fonttitle=\bfseries,top=2pt,bottom=2pt}

% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

% \DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% \SetKwInput{kwDeclare}{Declare}

% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% \setcopyright{acmcopyright}
% \copyrightyear{2022}
% \acmYear{2022}
% \acmDOI{XXXXXXX.XXXXXXX}

% %% These commands are for a PROCEEDINGS abstract or paper.
% %\acmConference[ESEC/FSE 2022]{The 30th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering}{14 - 18 November, 2022}{Singapore}
% %
% %  Uncomment \acmBooktitle if th title of the proceedings is different
% %  from ``Proceedings of ...''!
% %
% %\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
% %  June 03--05, 2018, Woodstock, NY} 
% \acmPrice{15.00}
% \acmISBN{978-1-4503-XXXX-X/18/06}


% \settopmatter{printacmref=false} % Removes citation information below abstract
% \renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference information in first column
% \pagestyle{empty} % removes running headers

% %%
% %% Submission ID.
% %% Use this when submitting an article to a sponsored event. You'll
% %% receive a unique submission ID from the organizers
% %% of the event, and this ID should be used as the parameter to this command.
% %%\acmSubmissionID{123-A56-BU3}

% %%
% %% The majority of ACM publications use numbered citations and
% %% references.  The command \citestyle{authoryear} switches to the
% %% "author year" style.
% %%
% %% If you are preparing content for an event
% %% sponsored by ACM SIGGRAPH, you must use the "author year" style of
% %% citations and references.
% %% Uncommenting
% %% the next command will enable that style.
% %%\citestyle{acmauthoryear}

% %%
% %% end of the preamble, start of the body of the document source.
% \begin{document}

% \thispagestyle{empty}
% % \hfill
% % \begin{adjustbox}{angle=90} 
% % \begin{sidewaystable}[]
% \begin{table*}[t!]
% \centering
% \footnotesize
% % \renewcommand\arraystretch{1.3}
% \caption{The Scott-Knott ranks and Median(IQR) MRE of our model DaL and other models.}

% \resizebox{\linewidth}{!}{ % reSize the table
% \begin{tabular}{clll|ll|ll|ll|ll|ll} \toprule
% \multirow{2}{*}{System} & \multicolumn{1}{c}{\multirow{2}{*}{Size}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{HINNPerf}} & \multicolumn{2}{c}{\texttt{DeepPerf}} & \multicolumn{2}{c}{\texttt{Perf-AL}} & \multicolumn{2}{c}{\texttt{DECART}} & \multicolumn{2}{c}{\texttt{SPLConqueror}} \\ \cline{3-14}
%  & \multicolumn{1}{c}{} & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) \\ \hline
% \multirow{5}{*}{\textsc{Apache}} & $S_1$ & 4 & 21.86 (7.36) & 4 & 19.44 (10.53) & 3 & 20.19 (6.34) & 5 & 33.57 (11.34) & 6 & 19.44 (6.48) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{14.44 (0.00)} \\
%  & $S_2$ & 5 & 12.89 (9.54) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.93 (3.89)} & 2 & 9.79 (4.56) & 6 & 32.97 (6.24) & 7 & 9.77 (5.36) & 4 & 13.89 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & \textbf{1} & \textbf{7.01 (1.74)} & 2 & 7.98 (1.91) & 4 & 31.73 (4.66) & 5 & 8.07 (1.05) & 3 & 13.99 (0.00) \\
%  & $S_4$ & 2 & 6.87 (1.95) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.58 (1.04)} & 2 & 6.85 (1.60) & 5 & 30.67 (6.84) & 6 & 7.47 (0.72) & 4 & 13.84 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & \textbf{1} & \textbf{5.85 (0.99)} & 2 & 6.66 (1.61) & 5 & 30.45 (4.91) & 6 & 7.14 (0.89) & 4 & 14.07 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{BDB-C}} & $S_1$ & 5 & 83.60 (208.75) & 5 & 167.55 (144.47) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{43.66 (42.88)} & 4 & 82.38 (57.27) & 6 & 51.88 (45.91) & 2 & 86.86 (0.00) \\
%  & $S_2$ & 3 & 21.92 (17.91) & 2 & 21.45 (13.61) & 2 & 18.17 (8.11) & 4 & 73.99 (22.51) & \cellcolor{red!20}6 & \cellcolor{red!20}13.37 (7.25) & 5 & 162.91 (0.00) \\
%  & $S_3$ & 2 & 8.31 (7.52) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.50 (9.20)} & 3 & 12.47 (4.08) & 3 & 69.74 (4.33) & 5 & 7.56 (5.07) & 4 & 193.89 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}2 & \cellcolor{green!20}3.60 (4.50) & \textbf{1} & \textbf{4.86 (2.18)} & 2 & 9.06 (9.76) & 3 & 69.50 (2.49) & 5 & 5.17 (5.07) & 4 & 231.68 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & 3 & 4.04 (1.24) & 4 & 7.08 (8.03) & 5 & 69.29 (0.69) & 7 & 3.54 (1.92) & 6 & 296.68 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{BDB-J}} & $S_1$ & 3 & 5.37 (4.74) & 2 & 3.58 (1.74) & 3 & 2.98 (3.34) & 5 & 37.45 (2.45) & \cellcolor{red!20}6 & \cellcolor{red!20}2.36 (0.75) & 4 & 12.29 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & \textbf{1} & \textbf{1.96 (0.36)} & 2 & 1.91 (0.68) & 4 & 37.90 (1.67) & 5 & 1.84 (0.17) & 3 & 24.85 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & 2 & 1.75 (0.41) & 3 & 2.01 (1.10) & 5 & 37.19 (1.70) & 6 & 1.64 (0.24) & 4 & 25.88 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & 2 & 1.52 (0.24) & 3 & 1.70 (0.37) & 5 & 37.74 (2.59) & 6 & 1.47 (0.12) & 4 & 29.01 (0.00) \\
%  & $S_5$ & \textbf{1} & \textbf{1.40 (0.34)} & 2 & 1.48 (0.32) & 3 & 1.69 (0.48) & 5 & 35.76 (4.47) & \cellcolor{red!20}6 & \cellcolor{red!20}1.37 (0.26) & 4 & 29.88 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{kanzi}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & 2 & 262.27 (175.07) & \textbf{1} & \textbf{196.36 (122.61)} & 3 & 1434.70 (1328.18) & 5 & 276.50 (272.43) & 4 & 2528.40 (0.00) \\
%  & $S_2$ & 2 & 95.31 (51.34) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{80.53 (51.36)} & 3 & 107.12 (43.75) & 4 & 961.11 (877.82) & 5 & 126.50 (142.62) & 4 & 1191.03 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}2 & \cellcolor{green!20}59.30 (38.47) & \textbf{1} & \textbf{62.20 (14.07)} & 2 & 68.62 (30.41) & 4 & 280.93 (147.45) & 6 & 74.08 (32.14) & 5 & 1059.28 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & \textbf{1} & \textbf{46.48 (19.58)} & 2 & 62.65 (26.54) & 4 & 266.53 (179.59) & 6 & 67.83 (15.79) & 5 & 1030.25 (0.00) \\
%  & $S_5$ & \textbf{1} & \textbf{35.29 (17.13)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{34.27 (11.87)} & 2 & 49.42 (9.99) & 4 & 169.12 (64.60) & 6 & 67.27 (17.95) & 5 & 1007.23 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{SQLite}} & $S_1$ & \textbf{1} & \textbf{73.52 (20.40)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{70.76 (27.86)} & \textbf{1} & \textbf{79.49 (25.36)} & 3 & 573.26 (340.38) & 4 & 74.14 (17.98) & 2 & 157.09 (0.00) \\
%  & $S_2$ & \textbf{1} & \textbf{76.41 (16.66)} & 2 & 76.69 (23.32) & 2 & 77.75 (22.47) & 3 & 386.74 (323.30) & \cellcolor{red!20}4 & \cellcolor{red!20}76.20 (22.74) & 2 & 84.41 (0.00) \\
%  & $S_3$ & \textbf{1} & \textbf{71.63 (11.58)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{71.02 (17.30)} & \textbf{1} & \textbf{75.01 (15.58)} & 2 & 424.32 (311.00) & 3 & 74.16 (20.12) & \textbf{1} & \textbf{75.72 (0.00)} \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & 2 & 70.84 (10.38) & 3 & 72.45 (12.11) & 4 & 363.18 (415.63) & 5 & 71.57 (14.72) & 2 & 69.61 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & 3 & 70.15 (9.71) & 4 & 72.87 (8.86) & 5 & 212.19 (295.12) & 6 & 68.51 (8.54) & 2 & 67.78 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{x264}} & $S_1$ & 4 & 10.21 (4.35) & 3 & 8.44 (2.69) & 2 & 8.04 (3.06) & 5 & 37.00 (9.43) & 6 & 9.27 (2.11) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.01 (0.00)} \\
%  & $S_2$ & \cellcolor{green!20}2 & \cellcolor{green!20}2.72 (1.52) & \textbf{1} & \textbf{2.77 (1.07)} & 2 & 3.17 (1.00) & 5 & 34.98 (7.81) & 6 & 6.29 (1.72) & 4 & 6.64 (0.00) \\
%  & $S_3$ & 2 & 1.57 (1.52) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.37 (0.46)} & 2 & 2.23 (0.90) & 5 & 36.25 (7.73) & 6 & 4.57 (1.03) & 4 & 6.31 (0.00) \\
%  & $S_4$ & 2 & 1.30 (1.17) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.81 (0.28)} & 3 & 1.74 (0.98) & 6 & 36.41 (6.47) & 7 & 3.66 (1.42) & 5 & 6.32 (0.00) \\
%  & $S_5$ & 2 & 0.96 (0.79) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.58 (0.15)} & 3 & 1.44 (0.90) & 6 & 36.20 (3.75) & 7 & 2.15 (1.05) & 5 & 6.36 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{Dune}} & $S_1$ & 3 & 9.37 (1.15) & 2 & 7.98 (0.98) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.86 (0.93)} & 5 & 55.73 (0.12) & 6 & \texttimes & 4 & 13.05 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & 2 & 6.15 (0.40) & \textbf{1} & \textbf{6.01 (0.21)} & 4 & 55.72 (0.53) & 5 & \texttimes & 3 & 13.09 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & 2 & 5.48 (0.39) & 2 & 5.52 (0.34) & 4 & 55.53 (1.69) & 5 & \texttimes & 3 & 13.10 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & 2 & 5.12 (0.38) & 3 & 5.26 (0.31) & 5 & 54.58 (1.48) & 6 & \texttimes & 4 & 13.16 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & 2 & 4.98 (0.64) & 3 & 5.15 (0.34) & 5 & 34.53 (21.14) & 6 & \texttimes & 4 & 13.17 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{HIPA$^{cc}$}} & $S_1$ & \textbf{1} & \textbf{7.50 (1.42)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.40 (1.05)} & 2 & 9.70 (1.28) & 4 & 31.99 (0.06) & 5 & \texttimes & 3 & 16.68 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & 2 & 4.53 (0.48) & 3 & 6.89 (1.44) & 5 & 31.98 (0.06) & 6 & \texttimes & 4 & 16.96 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & 2 & 3.67 (0.28) & 3 & 4.68 (0.90) & 5 & 31.99 (0.06) & 6 & \texttimes & 4 & 17.18 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & 2 & 2.70 (0.18) & 3 & 3.58 (1.00) & 5 & 31.98 (0.06) & 6 & \texttimes & 4 & 17.42 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & 2 & 2.23 (0.23) & 3 & 2.82 (0.57) & 5 & 31.97 (0.14) & 6 & \texttimes & 4 & 17.69 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{HSMGP}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & 2 & 5.03 (2.56) & 4 & 7.09 (3.04) & 5 & 66.70 (1294.05) & 6 & \texttimes & 3 & 15.04 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & 2 & 3.13 (0.49) & 3 & 3.69 (0.61) & 5 & 66.67 (0.11) & 6 & \texttimes & 4 & 22.63 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & 2 & 2.34 (0.38) & 2 & 2.28 (0.37) & 4 & 66.63 (0.18) & 5 & \texttimes & 3 & 32.46 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & 2 & 2.19 (0.23) & 3 & 2.23 (0.39) & 5 & 66.63 (0.14) & 6 & \texttimes & 4 & 33.74 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & 2 & 2.09 (0.25) & 3 & 1.94 (0.63) & 5 & 66.59 (0.20) & 6 & \texttimes & 4 & 35.86 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{Lrzip}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{31.88 (10.96)} & 3 & 41.97 (12.02) & 2 & 35.40 (16.59) & 4 & 58.45 (0.12) & 5 & \texttimes & 4 & 123.70 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & 3 & 24.10 (19.98) & 2 & 21.46 (4.53) & 4 & 58.46 (0.18) & 6 & \texttimes & 5 & 171.85 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & 3 & 23.71 (16.49) & 2 & 18.68 (3.20) & 4 & 58.44 (0.21) & 6 & \texttimes & 5 & 177.61 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & 3 & 19.82 (16.76) & 2 & 15.55 (1.71) & 4 & 58.48 (0.21) & 6 & \texttimes & 5 & 208.08 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & 3 & 10.39 (2.92) & 2 & 10.17 (0.91) & 4 & 58.39 (0.21) & 6 & \texttimes & 5 & 236.48 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{nginx}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & 2 & 8.08 (2.89) & 3 & 8.76 (4.10) & 5 & 1553.44 (965.63) & 6 & \texttimes & 4 & 574.23 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & 2 & 6.95 (1.74) & 2 & 6.15 (4.17) & 4 & 1637.60 (430.94) & 5 & \texttimes & 3 & 566.42 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & 3 & 6.46 (1.41) & 2 & 4.42 (1.44) & 5 & 1692.49 (305.78) & 6 & \texttimes & 4 & 567.41 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & 3 & 6.01 (1.68) & 2 & 4.09 (2.27) & 5 & 1784.76 (274.62) & 6 & \texttimes & 4 & 568.88 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & 3 & 7.27 (2.31) & 2 & 3.17 (1.72) & 5 & 1579.37 (515.54) & 6 & \texttimes & 4 & 563.91 (0.00) \\ \hline
% \multirow{5}{*}{\textsc{VP8}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & \textbf{1} & \textbf{1.72 (0.25)} & 2 & 4.68 (3.27) & 4 & 60.05 (2.03) & 5 & \texttimes & 3 & 29.39 (0.00) \\
%  & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & 2 & 1.27 (0.15) & 3 & 2.39 (1.21) & 5 & 60.04 (0.24) & 6 & \texttimes & 4 & 35.34 (0.00) \\
%  & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & 2 & 1.25 (0.14) & 3 & 1.93 (0.72) & 5 & 60.02 (0.29) & 6 & \texttimes & 4 & 36.26 (0.00) \\
%  & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & 2 & 1.15 (0.11) & 3 & 1.54 (0.40) & 5 & 59.99 (0.27) & 6 & \texttimes & 4 & 36.21 (0.00) \\
%  & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & 2 & 1.12 (0.11) & 3 & 1.45 (0.23) & 5 & 59.95 (0.68) & 6 & \texttimes & 4 & 37.14 (0.00) \\ \hline
% \multicolumn{2}{c}{Average $r$} & 1.48 &  & 1.95 &  & 2.4 &  & 4.5 &  & 5.72 &  & 3.73 & 
% \\
% \bottomrule
% \end{tabular}
% }
% % \label{tb:scott-knott}
% % \end{sidewaystable}
% \end{table*}
% % \end{adjustbox}
% % \hfill
% \end{document}
% \endinput
% %%
% %% End of file `sample-sigconf.tex'.


==> Tables/alg2-knee.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	\footnotesize
	
	\caption{Pseudo code of \textsc{AdaptingDepth}}
	\label{alg:adapt-code}
	\KwIn{A trained CART model $\mathcal{T}$}
     \KwOut{The most balanced $d$ value}
    %\KwOut{A set of division-dedicated models $\mathbfcal{M}$}
	%\kwDeclare{$\Delta=0.1$; bounds of weight: $w_{max}=10^3$; $w_{min}=0$}
      $d_j=0$\\
       \tcc{\textcolor{blue}{step 1.}}
      \While{$d_j\leq d_{max}$ from $\mathcal{T}$}{
          $\mathbfcal{D'}\leftarrow \emptyset$\\
           \If{$d_j<d$}
           {
             $\mathbfcal{D'}\leftarrow$ extract all the leaf divisions of samples from $\mathcal{T}$ at the $d_j$th depth\\
           }
           \Else{
              $\mathbfcal{D'}\leftarrow$ extract all divisions of samples from $\mathcal{T}$ at the $d_j$th depth\\
           }
           $d_j=d_j+1$\\
            \For{$\forall D_i \in \mathbfcal{D'}$} {
             calculate $z_1$ and $z_2$ for $D_i$ according to Equation~\ref{eq:adapt}\\
             $\mathbfcal{A}\leftarrow <D_i,d_j>$\\
            }
      }
      
        \tcc{\textcolor{blue}{step 2.}}
	  $\mathbfcal{N}\leftarrow$ extract the non-dominated divisions with respect to $z_1$ and $z_2$ from $\mathbfcal{A}$\\
      
      \If{$|\mathbfcal{N}|=1$} {
         \Return $d_j \leftarrow <D_i,d_j> \in \mathbfcal{N}$\\
      }
      \If{$|\mathbfcal{N}|=2$} {
         \Return the smaller $d_j \leftarrow <D_i,d_j> \in \mathbfcal{N}$\\
      }
      \tcc{\textcolor{blue}{step 3.}}
      $pd_{max}$ = 0\\
      find extreme points $D_{z_1}$ and $D_{z_2}$ in $\mathbfcal{N}$\\
        \For{$\forall <D_i,d_j> \in \mathbfcal{N}$} {
        $pd(D_i, \ell)=$ calculate the distance of $D_i$ to $\ell$ using Equation~\ref{eq:knee} with respect to $D_{z_1}$ and $D_{z_2}$\\
         \If{$pd(D_i, \ell) > pd_{max}$} {
         $pd_{max} = pd(D_i, \ell)$\\
         $\mathbfcal{C}=\emptyset$\\
         $\mathbfcal{C}\leftarrow<D_i,d_j>$\\
         }
        \ElseIf{$pd(D_i, \ell) = pd_{max}$} {
         $\mathbfcal{C}\leftarrow<D_i,d_j>$\\
         }
        }

\tcc{\textcolor{blue}{step 4.}}
$\mathbf{\overline{d}} =$ find the $d$ values with the most count of associated divisions from $\mathbfcal{C}$\\
        

       \If{$|\mathbf{\overline{d}}|=1$} {
         \Return $d_j \in \mathbf{\overline{d}}$\\
      } \Else{
      \Return the smallest $d_j \in \mathbf{\overline{d}}$\\
      }
   
       
	
\end{algorithm}

==> Tables/alg3.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	\footnotesize
	
	\caption{Pseudo code of predicting in \Model}
	\label{alg:phase3}
	\KwIn{The set of division-dedicated models $\mathbfcal{M}$; $\mathbfcal{D}$ extracted divisions of data samples; a new configuration $c$ to be predicted.}
    \KwOut{The predicted performance of $c$}
	\kwDeclare{Random Forest model $\mathcal{F}$}
	
	\If{$\mathcal{F}$ has not bee trained}
	{
	$\mathbfcal{U}\leftarrow$ Removing performance data and labeling the configurations based on their divisions in $\mathbfcal{D}$\\
	$\mathcal{F}\leftarrow$\textsc{trainRandomForest($\mathbfcal{U}$)}
	}
	
    $\mathcal{D}=$  \textsc{predict($\mathcal{F}$,$c$)}\\
    $\mathcal{M}=$ get the model from $\mathbfcal{M}$ that corresponds to the predicted division $\mathcal{D}$\\ 
       
    

    \Return \textsc{predict($\mathcal{M}$,$c$)}\\
	
\end{algorithm}

==> Tables/compare_models_bk.tex <==

% \begin{table*}[]
% \centering
% \footnotesize
% \caption{The Scott-Knott scores on the MRE of all evaluated models. The \colorbox{green!20}{cells} mean \Model has the highest score among all the models}
\begin{tabular}{P{1cm}P{1cm}P{1cm}P{1cm}|P{1cm}P{1cm}|P{1cm}P{1cm}|P{1cm}P{1cm}|P{1cm}P{1cm}|P{1cm}P{1cm}|P{1cm}P{1cm}}
\toprule

\textbf{System} &
   &
  \textbf{\Model} &
  \textbf{rDNN} &
  \textbf{\Model$_{RF}$} &
  \textbf{RF} &
  \textbf{\Model$_{CART}$} &
  \textbf{{CART}} &
  \textbf{\Model$_{LR}$} &
  \textbf{LR} &
  \textbf{\Model$_{SVR}$} &
  \textbf{SVR} &
  \textbf{\Model$_{KRR}$} &
  \textbf{KRR} &
  \textbf{\Model$_{kNN}$} &
  \textbf{$k$NN} \\ \midrule
\multirow{5}{*}{\textsc{Apache}}      & Size 1 & \cellcolor{green!20}\textbf{1} & 2 & \cellcolor{green!20}\textbf{1}& 3 & 2 & 2 & \cellcolor{green!20}\textbf{1} & 5  & 4 & 4  & 6  & 7  & 2  & 2  \\
                                      & Size 2 & 2          & \cellcolor{green!20}\textbf{1}& 2 & 2 & 2 & \cellcolor{green!20}\textbf{1}& 3  & 5  & 6 & 7  & 8  & 9  & 4  & 6  \\
                                      & Size 3 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 2 & 4 & 4 & \cellcolor{green!20}\textbf{1} & 7  & 6 & 9  & 10 & 11 & 5  & 8  \\
                                      & Size 4 & 2          & 2 & 3 & 2 & 5 & 4 & \cellcolor{green!20}\textbf{1} & 8  & 7 & 9  & 10 & 11 & 6  & 8  \\
                                      & Size 5 & 2          & 4 & 4 & 3 & 5 & 5 & \cellcolor{green!20}\textbf{1} & 9  & 7 & 10 & 11 & 12 & 6  & 8  \\ \hline
\multirow{5}{*}{\textsc{BDB-C}}       & Size 1 & 2          & 2 & 2 & 6 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 3  & 8  & 3 & 4  & 2  & 7  & 3  & 5  \\
                                      & Size 2 & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1}& 3 & 4 & \cellcolor{green!20}\textbf{1}& 2 & 7  & 6  & 5 & 5  & 4  & 6  & 5  & 6  \\
                                      & Size 3 & 2          & 5 & 4 & 4 & 3 & \cellcolor{green!20}\textbf{1}& 6  & 9  & 8 & 7  & 6  & 9  & 8  & 9  \\
                                      & Size 4 & \cellcolor{green!20}\textbf{1} & 3 & 3 & 4 & \cellcolor{green!20}\textbf{1}& 2 & 5  & 9  & 6 & 6  & 5  & 8  & 6  & 7  \\
                                      & Size 5 & \cellcolor{green!20}\textbf{1} & 3 & 2 & 4 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 4  & 9  & 6 & 7  & 5  & 9  & 6  & 8  \\ \hline
\multirow{5}{*}{\textsc{BDB-J}}       & Size 1 & 2          & 2 & 2 & 3 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 9  & 8  & 6 & 4  & 3  & 7  & 5  & 5  \\
                                      & Size 2 & 4          & 3 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 3 & 2 & 4  & 10 & 8 & 5  & 4  & 9  & 6  & 7  \\
                                      & Size 3 & 2          & 3 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 2 & 2 & 3  & 8  & 6 & 5  & 3  & 7  & 4  & 4  \\
                                      & Size 4 & 2          & 4 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 3 & 3 & 4  & 9  & 8 & 8  & 5  & 9  & 7  & 6  \\
                                      & Size 5 & 2          & 4 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 3 & 3 & 4  & 9  & 7 & 8  & 5  & 9  & 6  & 6  \\ \hline
\multirow{5}{*}{\textsc{x264}}        & Size 1 & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1}& 3 & 2 & 3 & 3 & 4  & 5  & 5 & 9  & 8  & 6  & 4  & 7  \\
                                      & Size 2 & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1}& 3 & 3 & 3 & 3 & 2  & 4  & 7 & 9  & 4  & 5  & 6  & 8  \\
                                      & Size 3 & \cellcolor{green!20}\textbf{1} & 2 & 5 & 5 & 4 & 4 & 2  & 5  & 6 & 9  & 5  & 7  & 8  & 9  \\
                                      & Size 4 & \cellcolor{green!20}\textbf{1} & 2 & 5 & 6 & 3 & 4 & 3  & 7  & 7 & 10 & 6  & 8  & 9  & 11 \\
                                      & Size 5 & \cellcolor{green!20}\textbf{1} & 2 & 5 & 6 & 3 & 4 & 6  & 8  & 8 & 11 & 7  & 9  & 10 & 12 \\ \hline
\multirow{5}{*}{\textsc{HSMGP}}       & Size 1 & \cellcolor{green!20}\textbf{1} & 8 & 6 & 5 & 7 & 7 & 2  & 11 & 4 & 5  & 3  & 10 & 8  & 9  \\
                                      & Size 2 & \cellcolor{green!20}\textbf{1} & 2 & 5 & 6 & 8 & 8 & 2  & 10 & 7 & 8  & 4  & 10 & 9  & 9  \\
                                      & Size 3 & \cellcolor{green!20}\textbf{1} & 2 & 4 & 5 & 7 & 7 & 2  & 10 & 6 & 9  & 3  & 10 & 8  & 8  \\
                                      & Size 4 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 4 & 7 & 8 & 4  & 11 & 6 & 10 & 5  & 11 & 9  & 9  \\
                                      & Size 5 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 3 & 7 & 6 & 10 & 9  & 4 & 8  & 5  & 10 & 9  & 9  \\ \hline
\multirow{5}{*}{\textsc{HIPA$^{cc}$}} & Size 1 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 3 & 4 & 4 & 9  & 8  & 5 & 7  & 4  & 9  & 6  & 8  \\
                                      & Size 2 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 3 & 3 & 3 & 6  & 10 & 5 & 6  & 5  & 8  & 4  & 7  \\
                                      & Size 3 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 3 & 3 & 3 & 5  & 11 & 5 & 8  & 6  & 10 & 4  & 9  \\
                                      & Size 4 & \cellcolor{green!20}\textbf{1} & 2 & 4 & 4 & 3 & 3 & 8  & 11 & 7 & 10 & 8  & 11 & 6  & 5  \\
                                      & Size 5 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 2 & 2 & 2 & 10 & 12 & 7 & 8  & 9  & 11 & 5  & 6  \\ \hline
\multirow{5}{*}{\textsc{VP8}}         & Size 1 & \cellcolor{green!20}\textbf{1} & 5 & 4 & 6 & 2 & 3 & 5  & 7  & 9 & 10 & 7  & 12 & 10 & 11 \\
                                      & Size 2 & 4          & 5 & 3 & 4 & \cellcolor{green!20}\textbf{1}& 2 & 4  & 8  & 6 & 11 & 7  & 12 & 9  & 10 \\
                                      & Size 3 & \cellcolor{green!20}\textbf{1} & 2 & 2 & 2 & 2 & 3 & 5  & 11 & 5 & 9  & 6  & 10 & 8  & 8  \\
                                      & Size 4 & \cellcolor{green!20}\textbf{1} & 2 & 2 & 2 & 2 & 2 & 3  & 8  & 4 & 6  & 3  & 7  & 5  & 6  \\
                                      & Size 5 & \cellcolor{green!20}\textbf{1} & 2 & 3 & 4 & 2 & 3 & 6  & 12 & 7 & 10 & 5  & 11 & 8  & 9  \\ \hline
\multirow{5}{*}{\textsc{Lrzip}}       & Size 1 & 3          & 4 & 2 & 3 & \cellcolor{green!20}\textbf{1}& 2 & 5  & 10 & 5 & 5  & 7  & 9  & 6  & 5  \\
                                      & Size 2 & 3          & 4 & 2 & 2 & \cellcolor{green!20}\textbf{1}& 2 & 5  & 8  & 6 & 6  & 7  & 9  & 5  & 5  \\
                                      & Size 3 & 3          & 4 & 2 & \cellcolor{green!20}\textbf{1}& \cellcolor{green!20}\textbf{1}& 2 & 6  & 9  & 7 & 6  & 8  & 10 & 5  & 5  \\
                                      & Size 4 & 3          & 4 & 4 & 7 & \cellcolor{green!20}\textbf{1}& 2 & 8  & 10 & 2 & 3  & 6  & 9  & 5  & 8  \\
                                      & Size 5 & 3          & 4 & \cellcolor{green!20}\textbf{1}& 3 & \cellcolor{green!20}\textbf{1}& 2 & 7  & 9  & 7 & 8  & 9  & 11 & 5  & 6  \\ \midrule
Average &
   &
  \cellcolor{green!20}\textbf{1.63} &
  2.78 &
  2.90 &
  3.38 &
  2.95 &
  3.15 &
  4.63 &
  8.58 &
  6.00 &
  7.48 &
  5.85 &
  9.13 &
  6.25 &
  7.35
\\ \bottomrule






% System            & Size & \Model                              & DNN & \Model$_{RF}$ & RF  & \Model$_{CART}$ & DT  & \Model$_{LR}$ & LR & \Model$_{SVR}$ & SVR & \Model$_{KRR}$ & KRR & \Model$_{kNN}$ & KNN \\ \midrule
%                          & 9   & -                                   & -  & -  & -  & -  & -  & -  & - & -  & - & - & - & - & - \\
%                          & 18  & 8                                   & 9  & 8  & 8  & 8  & 9  & 7  & 5 & 4  & 3 & 2 & \cellcolor{green!20}\textbf{1}& 6 & 4 \\
%                          & 27  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 9  & 10 & 8  & 8  & 11 & 5 & 6  & 3 & 2 & \cellcolor{green!20}\textbf{1}& 7 & 4 \\
%                          & 36  & 10                                  & 10 & 9  & 10 & 7  & 8  & 11 & 4 & 5  & 3 & 2 & \cellcolor{green!20}\textbf{1}& 6 & 4 \\ 
% \multirow{-5}{*}{\textsc{Apache}} & 45  & 11                                  & 9  & 9  & 10 & 8  & 8  & 12 & 4 & 6  & 3 & 2 & \cellcolor{green!20}\textbf{1}& 7 & 5 \\ \hline
%                          & 18  & 7                                   & 8  & 7  & 3  & 9  & 8  & 6  & \cellcolor{green!20}\textbf{1}& 6  & 5 & 7 & 2 & 6 & 4 \\
%                          & 36  & 7                                   & 8  & 6  & 5  & 7  & 7  & \cellcolor{green!20}\textbf{1} & 2 & 4  & 4 & 5 & 3 & 4 & 3 \\
%                          & 54  & 9                                   & 6  & 7  & 7  & 8  & 10 & 4  & \cellcolor{green!20}\textbf{1}& 3  & 4 & 5 & 2 & 3 & 2 \\
%                          & 72  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{9}  & 7  & 7  & 6  & 9  & 8  & 5  & \cellcolor{green!20}\textbf{1}& 4  & 4 & 5 & 2 & 4 & 3 \\
% \multirow{-5}{*}{\textsc{BDB-C}}   & 90  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{10} & 8  & 9  & 7  & 10 & 10 & 6  & \cellcolor{green!20}\textbf{1}& 5  & 4 & 6 & 2 & 5 & 3 \\ \hline
%                          & 26  & 8                                   & 8  & 8  & 7  & 9  & 9  & \cellcolor{green!20}\textbf{1} & 2 & 4  & 6 & 7 & 3 & 5 & 5 \\
%                          & 52  & 7                                   & 8  & 11 & 11 & 9  & 10 & 7  & \cellcolor{green!20}\textbf{1}& 3  & 6 & 7 & 2 & 5 & 4 \\
%                          & 78  & 7                                   & 6  & 8  & 8  & 7  & 7  & 6  & \cellcolor{green!20}\textbf{1}& 3  & 4 & 6 & 2 & 5 & 5 \\
%                          & 104 & 9                                   & 7  & 10 & 10 & 8  & 8  & 6  & \cellcolor{green!20}\textbf{1}& 3  & 3 & 6 & 2 & 4 & 5 \\
% \multirow{-5}{*}{\textsc{BDB-J}}   & 130 & 9                                   & 7  & 10 & 10 & 8  & 8  & 6  & \cellcolor{green!20}\textbf{1}& 4  & 3 & 6 & 2 & 5 & 5 \\ \hline
%                          & 16  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{9}  & 9  & 7  & 8  & 7  & 7  & 6  & 5 & 5  & \cellcolor{green!20}\textbf{1}& 2 & 4 & 6 & 3 \\
%                          & 32  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{9}  & 9  & 7  & 7  & 7  & 7  & 8  & 6 & 3  & \cellcolor{green!20}\textbf{1}& 6 & 5 & 4 & 2 \\
%                          & 48  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{9}  & 8  & 5  & 5  & 6  & 6  & 7  & 4 & 4  & \cellcolor{green!20}\textbf{1}& 5 & 3 & 2 & \cellcolor{green!20}\textbf{1}\\
%                          & 64  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 7  & 6  & 9  & 8  & 8  & 4 & 5  & 2 & 6 & 4 & 3 & \cellcolor{green!20}\textbf{1}\\
% \multirow{-5}{*}{\textsc{x264}}   & 80  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{12} & 11 & 8  & 7  & 10 & 9  & 6  & 4 & 5  & 2 & 6 & 4 & 3 & \cellcolor{green!20}\textbf{1}\\ \hline
%                          & 77  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 4  & 6  & 7  & 5  & 5  & 10 & \cellcolor{green!20}\textbf{1}& 8  & 7 & 9 & 2 & 4 & 3 \\
%                          & 173 & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 7  & 6  & 4  & 4  & 9  & \cellcolor{green!20}\textbf{1}& 5  & 4 & 8 & 2 & 3 & 3 \\
%                          & 384 & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 8  & 7  & 5  & 5  & 9  & \cellcolor{green!20}\textbf{1}& 6  & 3 & 9 & 2 & 4 & 4 \\
% \multirow{-4}{*}{\textsc{HSMGP}}  & 480  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{12}  & 11  & 10     & 9   & 6      & 5   & 8      & \cellcolor{green!20}\textbf{1} & 7       & 3   & 8       & 2   & 4       & 3   \\ \hline
%                          & 261 & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 9  & 9  & 8  & 8  & \cellcolor{green!20}\textbf{1} & 2 & 7  & 5 & 8 & 3 & 6 & 4 \\
%                          & 528 & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{10} & 9  & 8  & 8  & 8  & 8  & \cellcolor{green!20}\textbf{1} & 2 & 6  & 5 & 6 & 3 & 7 & 4 \\
%                          & 736 & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 9  & 9  & 9  & 9  & 5  & \cellcolor{green!20}\textbf{1}& 7  & 4 & 6 & 2 & 8 & 3 \\
% \multirow{-4}{*}{\textsc{HIPA$_{cc}$}} & 1281 & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{12}  & 11  & 9      & 9   & 10     & 10  & 4      & \cellcolor{green!20}\textbf{1} & 6       & 3   & 5       & 2   & 7       & 8   \\ \hline
%                          & 13  & 5                                   & 5  & 6  & 4  & 6  & 5  & 3  & \cellcolor{green!20}\textbf{1}& 5  & \cellcolor{green!20}\textbf{1}& 4 & 2 & 5 & 3 \\
%                          & 26  & 7                                   & 8  & 7  & 6  & 8  & 7  & 6  & 2 & 4  & \cellcolor{green!20}\textbf{1}& 6 & 3 & 5 & 4 \\
%                          & 39  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{11} & 10 & 10 & 8  & 10 & 9  & 7  & \cellcolor{green!20}\textbf{1}& 6  & 2 & 7 & 3 & 5 & 4 \\
%                          & 52  & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{8}  & 8  & 7  & 7  & 7  & 7  & 6  & \cellcolor{green!20}\textbf{1}& 5  & 3 & 6 & 2 & 4 & 3 \\
% \multirow{-5}{*}{\textsc{VP8}}    & 65   & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{13}  & 10  & 11     & 9   & 12     & 11  & 7      & \cellcolor{green!20}\textbf{1} & 6       & 3   & 8       & 2   & 5       & 4   \\ \hline
%                          & 12  & 9                                   & 2  & 8  & 3  & 6  & 4  & 6  & \cellcolor{green!20}\textbf{1}& 10 & 5 & 7 & 2 & 8 & 4 \\
%                          & 24  & 8                                   & 5  & 6  & 3  & 8  & 8  & 4  & \cellcolor{green!20}\textbf{1}& 9  & 7 & 6 & 2 & 7 & 4 \\
%                          & 36  & 8                                   & 5  & 7  & 4  & 9  & 9  & 4  & \cellcolor{green!20}\textbf{1}& 10 & 8 & 6 & 2 & 7 & 3 \\
%                          & 48  & 7                                   & 5  & 6  & 4  & 9  & 9  & 3  & \cellcolor{green!20}\textbf{1}& 8  & 7 & 5 & 2 & 5 & 3 \\
% \multirow{-5}{*}{\textsc{Lrzip}}  & 60  & 8                                   & 5  & 7  & 4  & 9  & 9  & 3  & \cellcolor{green!20}\textbf{1}& 7  & 6 & 4 & 2 & 5 & 3 \\ \hline
% Total              &      & \cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\cellcolor{green!20}\textbf{345} & 296 & 293    & 261 & 293    & 287 & 220    & 74 & 204     & 139 & 211     & 86  & 189     & 131 \\ \bottomrule
\end{tabular}
% \label{tb:scott-knott}
% \end{table*}


==> Tables/compare_models_old.tex <==

% \begin{table*}[]
% \centering
% \footnotesize
% \caption{The Scott-Knott scores on the MRE of all evaluated models. The \colorbox{green!20}{cells} mean \Model has the highest score among all the models}
\setlength{\tabcolsep}{0.9mm}
\begin{tabular}{cc|cccc|cccc|cccc|cccc|cccc|cccc|cccc}
\toprule

\multirow{2}{*}{\textbf{System}} &
   &
  \multicolumn{2}{c}{\textbf{\Model}} &
  \multicolumn{2}{c|}{\textbf{rDNN}} &
  \multicolumn{2}{c}{\textbf{\Model$_{RF}$}} &
  \multicolumn{2}{c|}{\textbf{RF}} &
  \multicolumn{2}{c}{\textbf{\Model$_{CART}$}} &
  \multicolumn{2}{c|}{\textbf{{CART}}} &
  \multicolumn{2}{c}{\textbf{\Model$_{LR}$}} &
  \multicolumn{2}{c|}{\textbf{LR}} &
  \multicolumn{2}{c}{\textbf{\Model$_{SVR}$}} &
  \multicolumn{2}{c|}{\textbf{SVR}} &
  \multicolumn{2}{c}{\textbf{\Model$_{KRR}$}} &
  \multicolumn{2}{c|}{\textbf{KRR}} &
  \multicolumn{2}{c}{\textbf{\Model$_{kNN}$}} &
  \multicolumn{2}{c}{\textbf{$k$NN}} \\  \cmidrule{3-30}

  &&\textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} &
  \textbf{$r$} &
  \textbf{M (IQR)} \\ \midrule


  \multirow{5}{*}{\textsc{Apache}}      & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

   & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

    & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

     & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

      & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\ \midrule

       \multirow{5}{*}{\textsc{Apache}}      & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

   & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

    & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

     & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\

      & $S_1$ & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1}& 41.8 (32.5) & 3 & 41.8 (32.5) & 2 & 41.8 (32.5) & 2 & 41.8 (32.5) & \cellcolor{green!20}\textbf{1} & 41.8 (32.5) & 5 & 41.8 (32.5)  & 4 & 41.8 (32.5) & 4 & 41.8 (32.5)  & 6 & 41.8 (32.5)  & 7 & 41.8 (32.5)  & 2 & 41.8 (32.5)  & 2 & 41.8 (32.5)  \\ \midrule
                                  

\end{tabular}
% \label{tb:scott-knott}
% \end{table*}


==> Tables/data_example.tex <==
% \begin{table}[]
% \centering
% \small
% \caption{An example of performance dataset. $\overline{x}$ are the configurations and $\varmathbb{P}$ is the performance value.}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
$x_{1}$ & $x_{2}$ & $x_{3}$ & $\cdots$ & $x_{n-2}$ & $x_{n-1}$ & $x_{n}$ & $\varmathbb{P}$ \\ \hline
0 & 0 & 0 & $\cdots$ & 0 & 3 & 10 & 1200 \\ 
0 & 1 & 0 & $\cdots$ & 0 & 2 & 11 & 2100 \\ 
$\cdots$        & $\cdots$  & $\cdots$       & $\cdots$       & $\cdots$       & $\cdots$ & $\cdots$ & $\cdots$ \\ 
0 & 0 & 1 & $\cdots$ & 0 & 9 & 23 & 1260 \\ 
0 & 0 & 1 & $\cdots$ & 1 & 8 & 65 & 1140 \\ \hline
\end{tabular}
% \label{tb:data_example}
% \end{table}

==> Tables/response_compare_clustering.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
\begin{tabular}{clllllllll||llll}
\toprule
\multirow{2}{*}{System} & \multicolumn{1}{c}{\multirow{2}{*}{Size}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{DBSCAN}} & \multicolumn{2}{c}{\texttt{Agglomerative}} & \multicolumn{2}{c}{\texttt{kMeans}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{DaL-FSE}} \\ \cline{3-14}
 & \multicolumn{1}{c}{} & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) \\ \hline
\multirow{5}{*}{\textsc{Apache}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.86 (7.36)} & 2 & 26.29 (15.23) & 3 & 30.99 (20.01) & 3 & 40.02 (22.13) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.86 (7.36)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{21.86 (7.36)} \\
 & $S_2$ & \cellcolor{green!20}2 & \cellcolor{green!20}12.89 (7.87) & 2 & 16.24 (10.00) & \textbf{1} & \textbf{15.45 (5.76)} & \textbf{1} & \textbf{14.85 (5.21)} & \textbf{1} & \textbf{12.89 (7.87)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{11.87 (9.22)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & 3 & 13.24 (9.29) & 2 & 10.62 (3.24) & 2 & 10.60 (6.77) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.56 (1.92)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.87 (1.95)} & 4 & 10.44 (4.15) & 3 & 8.63 (2.49) & 2 & 7.39 (2.84) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.87 (1.95)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.87 (1.95)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & 4 & 9.18 (3.33) & 3 & 7.82 (2.20) & 2 & 6.08 (2.53) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.78 (1.08)} \\ \hline
\multirow{5}{*}{\textsc{BDB-C}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{83.60 (208.75)} & 2 & 438.69 (291.46) & 2 & 361.68 (382.62) & 2 & 309.58 (359.65) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{83.60 (208.75)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{83.60 (208.75)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.92 (17.91)} & 3 & 170.67 (133.10) & 2 & 117.38 (99.35) & 3 & 145.13 (135.06) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.92 (17.91)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{21.92 (17.91)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.31 (7.52)} & 2 & 43.57 (70.53) & 2 & 39.10 (72.34) & 3 & 38.29 (56.01) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.31 (7.52)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.31 (7.52)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.60 (4.50)} & 2 & 29.43 (29.08) & 2 & 25.32 (26.66) & 3 & 23.07 (43.38) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.60 (4.50)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{3.60 (4.50)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & 3 & 33.50 (18.42) & 2 & 11.67 (13.49) & 4 & 19.27 (22.25) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.88 (1.24)} \\ \hline
\multirow{5}{*}{\textsc{BDB-J}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.37 (4.74)} & 2 & 14.51 (9.69) & 3 & 14.57 (22.68) & 3 & 11.03 (13.62) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.37 (4.74)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.37 (4.74)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & 2 & 6.58 (6.33) & 3 & 7.12 (20.32) & 2 & 3.08 (4.46) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.83 (0.45)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & 2 & 3.48 (0.94) & 3 & 2.24 (4.85) & 2 & 2.05 (0.47) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.58 (0.26)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & 3 & 2.53 (0.87) & 4 & 1.82 (0.68) & 2 & 1.76 (0.34) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.45 (0.22)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.40 (0.34)} & 3 & 2.61 (0.58) & 2 & 1.68 (0.26) & 2 & 1.62 (0.39) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.40 (0.34)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.40 (0.34)} \\ \hline
\multirow{5}{*}{\textsc{kanzi}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & 3 & 545.20 (418.67) & 3 & 553.75 (502.84) & 2 & 531.18 (334.99) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{196.15 (213.73)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{95.31 (51.34)} & 2 & 204.18 (138.71) & 3 & 196.73 (275.40) & 2 & 190.64 (148.79) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{95.31 (51.34)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{95.31 (51.34)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{59.30 (38.47)} & 2 & 160.72 (82.07) & 2 & 118.26 (106.12) & 2 & 119.90 (76.87) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{59.30 (38.47)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{59.30 (38.47)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & 3 & 103.18 (113.16) & 2 & 81.27 (28.15) & 2 & 81.88 (26.24) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{42.93 (18.75)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{35.29 (17.13)} & 4 & 91.90 (48.67) & 2 & 60.45 (19.99) & 3 & 65.93 (25.27) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{35.29 (17.13)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{35.29 (17.13)} \\ \hline
\multirow{5}{*}{\textsc{SQLite}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{73.52 (20.40)} & 2 & 87.19 (30.88) & 2 & 90.37 (22.58) & 2 & 98.63 (64.82) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{73.52 (20.40)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{73.52 (20.40)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{76.41 (16.66)} & 3 & 84.27 (33.49) & 2 & 81.43 (21.75) & 3 & 83.39 (34.67) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{76.41 (16.66)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{76.41 (16.66)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{71.63 (11.58)} & 3 & 86.71 (25.06) & 2 & 75.22 (13.79) & 2 & 73.63 (18.36) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{71.63 (11.58)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{71.63 (11.58)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & 3 & 81.04 (15.76) & 2 & 71.66 (12.67) & 2 & 75.77 (19.71) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{66.94 (10.61)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & 4 & 77.13 (17.36) & 2 & 71.44 (12.01) & 3 & 72.32 (13.70) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{64.20 (13.91)} \\ \hline
\multirow{5}{*}{\textsc{x264}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.21 (4.35)} & 2 & 15.09 (9.65) & 2 & 13.36 (12.90) & 3 & 15.72 (26.44) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.21 (4.35)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{10.21 (4.35)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.72 (1.52)} & 3 & 8.49 (6.80) & 2 & 5.44 (3.96) & 3 & 4.48 (3.51) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.72 (1.52)} & \textbf{1} & \textbf{2.74 (1.36)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.57 (1.52)} & 3 & 6.71 (4.70) & 2 & 2.15 (0.75) & 2 & 1.91 (1.69) & 2 & 1.57 (1.52) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.56 (0.70)} \\
 & $S_4$ & \textbf{1} & \textbf{1.30 (1.17)} & 2 & 7.28 (6.34) & \textbf{1} & \textbf{1.29 (0.80)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.05 (0.86)} & 2 & 1.30 (1.17) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.00 (0.56)} \\
 & $S_5$ & 3 & 0.96 (0.79) & 4 & 4.46 (4.53) & 2 & 0.83 (0.49) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.61 (0.33)} & 2 & 0.96 (0.79) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.60 (0.36)} \\ \hline
\multirow{5}{*}{\textsc{Dune}} & $S_1$ & \textbf{1} & \textbf{9.37 (1.15)} & 3 & 12.87 (3.21) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{9.21 (1.43)} & 2 & 9.42 (1.44) & \textbf{1} & \textbf{9.37 (1.15)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{9.19 (0.89)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & 4 & 13.56 (3.20) & 2 & 6.60 (0.64) & 3 & 6.92 (0.61) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.95 (0.54)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & 3 & 15.17 (3.61) & 2 & 6.14 (0.46) & 2 & 6.09 (0.56) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.81 (0.48)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & 3 & 20.52 (3.50) & 2 & 5.61 (0.63) & 2 & 5.52 (0.51) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.23 (0.35)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & 4 & 26.16 (4.58) & 2 & 4.98 (0.25) & 3 & 5.00 (0.31) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{3.98 (0.19)} \\ \hline
\multirow{5}{*}{\textsc{HIPA$^{cc}$}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.50 (1.42)} & 3 & 14.44 (7.83) & 2 & 9.95 (1.94) & 2 & 9.46 (1.37) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.50 (1.42)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.50 (1.42)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & 4 & 14.76 (3.76) & 3 & 5.61 (0.72) & 2 & 5.50 (0.63) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.48 (0.38)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & 4 & 10.33 (1.09) & 3 & 4.26 (0.44) & 2 & 4.18 (0.41) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{3.43 (0.34)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & 4 & 7.31 (0.65) & 3 & 2.95 (0.36) & 2 & 2.96 (0.18) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.60 (0.15)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & 4 & 6.92 (0.60) & 3 & 2.27 (0.14) & 2 & 2.20 (0.09) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.11 (0.08)} \\ \hline
\multirow{5}{*}{\textsc{HSMGP}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & 4 & 21.00 (94.17) & 2 & 10.21 (14.94) & 3 & 12.27 (47.67) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.14 (1.44)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & 4 & 2646.68 (2520.59) & 2 & 3.42 (3.02) & 3 & 5.47 (17.62) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.06 (0.19)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & 4 & 9923.71 (8468.77) & 2 & 2.31 (0.41) & 3 & 2.59 (0.72) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.42 (0.13)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & 4 & 14463.33 (8345.45) & 2 & 2.15 (0.51) & 3 & 2.30 (0.37) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.33 (0.08)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & 4 & 5104.04 (2486.94) & 2 & 1.80 (0.29) & 3 & 1.89 (0.22) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.19 (0.08)} \\ \hline
\multirow{5}{*}{\textsc{Lrzip}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{31.88 (10.96)} & 3 & 72.91 (33.63) & 2 & 38.43 (19.53) & 3 & 66.44 (35.18) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{31.88 (10.96)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{31.88 (10.96)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & 3 & 209.93 (186.42) & 2 & 23.70 (17.77) & 3 & 48.56 (93.35) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{10.51 (4.39)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & 4 & 288.22 (299.90) & 2 & 14.75 (16.26) & 3 & 32.91 (20.58) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.04 (2.37)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & 3 & 124.12 (186.64) & 2 & 12.59 (7.86) & 3 & 34.68 (46.30) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.95 (0.99)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & 3 & 110.41 (46.00) & 2 & 5.56 (4.32) & 4 & 22.75 (136.13) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.03 (0.26)} \\ \hline
\multirow{5}{*}{\textsc{nginx}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & 3 & 15.18 (10.27) & 2 & 7.30 (3.27) & 2 & 7.89 (4.12) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.11 (1.45)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & 3 & 7.83 (4.25) & 2 & 5.87 (1.00) & 2 & 5.52 (1.26) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.60 (1.14)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & 3 & 4.94 (3.79) & 2 & 5.23 (1.55) & 2 & 4.49 (1.57) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.14 (0.40)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & 2 & 3.75 (3.14) & 3 & 4.95 (1.01) & 3 & 4.19 (1.15) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.99 (0.47)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & 4 & 5.83 (2.09) & 2 & 4.10 (1.83) & 3 & 4.32 (1.20) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.98 (0.21)} \\ \hline
\multirow{5}{*}{\textsc{VP8}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & 4 & 7.58 (2.89) & 2 & 2.16 (1.08) & 3 & 2.86 (1.04) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.56 (0.18)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & 4 & 7.39 (2.36) & 3 & 1.45 (0.54) & 2 & 1.40 (0.16) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.15 (0.05)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & 4 & 9.02 (3.35) & 3 & 1.32 (0.32) & 2 & 1.25 (0.13) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.08 (0.04)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & 4 & 9.65 (3.27) & 3 & 1.31 (0.31) & 2 & 1.17 (0.09) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.98 (0.05)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & 4 & 10.23 (5.77) & 2 & 1.03 (0.12) & 3 & 1.05 (0.10) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.90 (0.06)} \\ \hline
\multicolumn{2}{c}{Average $r$} & 1.05 &  & 3.15 &  & 2.25 &  & 2.43 &  & 1.05 &  & 1 & 
\\
\bottomrule
\end{tabular}
% \end{table}

==> Tables/response_compare_ensemble.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t!]
% \footnotesize
% \setlength{\tabcolsep}{1.2mm}
% \renewcommand\arraystretch{1.3}
\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{p{1cm}lp{0.2cm}lp{0.2cm}lp{0.2cm}l||p{0.2cm}lp{0.2cm}lp{0.2cm}l||p{0.2cm}lp{0.2cm}lp{0.2cm}lp{0.2cm}l} \toprule
\multirow{2}{*}{System} & \multicolumn{1}{c}{\multirow{2}{*}{Size}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{Bagging$_{HINN}$}} & \multicolumn{2}{c}{\texttt{AdaBoost$_{HINN}$}} & \multicolumn{2}{c}{\texttt{DaL$_{LR}$}} & \multicolumn{2}{c}{\texttt{Bagging$_{LR}$}} & \multicolumn{2}{c}{\texttt{AdaBoost$_{LR}$}} & \multicolumn{2}{c}{\texttt{DaL$_{CART}$}} & \multicolumn{2}{c}{\texttt{RF}} & \multicolumn{2}{c}{\texttt{XGBoost}} & \multicolumn{2}{c}{\texttt{AdaBoost$_{CART}$}} \\  \cline{3-22}
 & \multicolumn{1}{c}{} & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) \\  \hline
\multirow{5}{*}{\textsc{Apache}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.86 (7.36)} & 3 & 24.64 (9.80) & 2 & 24.78 (6.66) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{19.71 (6.80)} & 2 & 20.81 (4.47) & 2 & 20.44 (5.03) & 2 & 21.61 (6.69) & 3 & 21.20 (7.72) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{19.03 (7.50)} & 4 & 24.06 (7.47) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.89 (7.87)} & \textbf{1} & \textbf{14.84 (6.31)} & \textbf{1} & \textbf{15.61 (5.39)} & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.77 (7.55)} & 3 & 17.64 (2.12) & 2 & 16.69 (2.45) & \cellcolor{green!20}2 & \cellcolor{green!20}10.12 (5.05) & 2 & 12.02 (6.58) & \textbf{1} & \textbf{10.70 (3.76)} & 3 & 13.82 (4.42) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & 2 & 11.20 (5.52) & 3 & 12.19 (10.08) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.42 (2.14)} & 2 & 16.11 (1.34) & 2 & 16.25 (1.68) & 2 & 9.10 (1.31) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.65 (1.46)} & 2 & 9.37 (1.36) & 2 & 9.04 (1.70) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.87 (1.95)} & 3 & 9.17 (23.67) & 2 & 9.86 (2.32) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.39 (1.16)} & 2 & 16.20 (0.82) & 2 & 15.96 (1.40) & 3 & 7.97 (1.35) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.63 (1.19)} & 4 & 8.70 (1.14) & 2 & 7.64 (0.99) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & 3 & 7.81 (24.03) & 2 & 8.90 (3.19) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.75 (0.55)} & 2 & 16.04 (1.37) & 2 & 16.18 (1.80) & 3 & 7.63 (1.00) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.43 (1.11)} & 4 & 8.17 (1.69) & 2 & 7.22 (0.97) \\ \hline
\multirow{5}{*}{\textsc{BDB-C}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{83.60 (208.75)} & \textbf{1} & \textbf{158.49 (97.21)} & 2 & 239.27 (165.36) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{65.09 (37.30)} & 3 & 485.41 (235.62) & 2 & 453.92 (139.97) & \textbf{1} & \textbf{47.20 (19.75)} & 4 & 253.78 (93.63) & \cellcolor{red!20}2 & \cellcolor{red!20}40.05 (54.70) & 3 & 211.60 (191.00) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.92 (17.91)} & 2 & 87.45 (64.92) & 3 & 175.89 (62.71) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{49.04 (47.11)} & 3 & 529.58 (158.69) & 2 & 565.28 (157.43) & 2 & 16.81 (8.59) & 3 & 73.41 (118.30) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{16.30 (4.99)} & 3 & 95.94 (19.68) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.31 (7.52)} & 2 & 52.55 (22.07) & 3 & 100.26 (43.36) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{29.00 (78.81)} & 2 & 460.89 (90.55) & 3 & 496.74 (56.61) & \cellcolor{green!20}2 & \cellcolor{green!20}6.72 (5.82) & 3 & 18.64 (19.42) & \textbf{1} & \textbf{10.23 (1.63)} & 4 & 43.94 (7.78) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.60 (4.50)} & 2 & 35.88 (17.56) & 3 & 77.71 (33.23) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{24.55 (4.18)} & 2 & 440.07 (77.70) & 3 & 475.09 (43.17) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.15 (2.78)} & 3 & 11.32 (6.77) & 2 & 8.51 (0.97) & 3 & 21.47 (5.45) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & 2 & 31.49 (17.12) & 3 & 58.63 (19.41) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{22.88 (3.78)} & 2 & 460.51 (88.56) & 3 & 473.16 (64.47) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.24 (3.09)} & 3 & 6.64 (3.35) & 2 & 7.50 (1.11) & 3 & 11.07 (2.28) \\ \hline
\multirow{5}{*}{\textsc{BDB-J}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.37 (4.74)} & 2 & 11.23 (6.65) & 2 & 14.06 (7.13) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.31 (2.96)} & 3 & 43.30 (6.44) & 2 & 40.89 (6.68) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.98 (0.81)} & 3 & 8.36 (10.48) & 2 & 7.39 (1.07) & \textbf{1} & \textbf{3.61 (2.31)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & 3 & 5.24 (33.48) & 2 & 5.17 (3.19) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.77 (0.49)} & 2 & 37.75 (5.70) & 3 & 39.84 (6.41) & 2 & 2.05 (0.33) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.82 (0.29)} & 3 & 6.10 (0.51) & \textbf{1} & \textbf{1.85 (0.20)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & 3 & 3.29 (1.29) & 2 & 3.75 (0.62) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.41 (0.46)} & 2 & 37.72 (3.80) & 2 & 38.85 (4.51) & 3 & 1.92 (0.27) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.57 (0.21)} & 4 & 5.71 (0.61) & 2 & 1.78 (0.25) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & 3 & 2.93 (0.80) & 2 & 2.70 (0.59) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.57 (0.66)} & 3 & 37.07 (3.03) & 2 & 36.17 (4.46) & 3 & 1.67 (0.29) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.43 (0.21)} & 4 & 5.48 (0.55) & 2 & 1.66 (0.21) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.40 (0.34)} & 3 & 2.48 (0.56) & 2 & 2.39 (0.38) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.23 (0.65)} & 3 & 37.27 (3.01) & 2 & 36.52 (5.25) & 3 & 1.67 (0.43) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.40 (0.23)} & 4 & 5.34 (0.42) & 2 & 1.55 (0.29) \\ \hline
\multirow{5}{*}{\textsc{kanzi}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & 2 & 256.87 (151.84) & 3 & 410.20 (187.36) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{551.03 (1244.41)} & \textbf{1} & \textbf{1158.20 (365.64)} & \textbf{1} & \textbf{1087.10 (248.90)} & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{178.67 (123.16)} & 2 & 359.19 (147.95) & \textbf{1} & \textbf{190.78 (98.22)} & 2 & 426.88 (221.92) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{95.31 (51.34)} & 2 & 184.70 (53.30) & 3 & 285.91 (71.88) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{383.06 (493.33)} & 3 & 1224.60 (377.56) & 2 & 1259.43 (331.27) & \textbf{1} & \textbf{86.55 (35.63)} & 2 & 155.50 (51.71) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{84.19 (30.01)} & 3 & 253.92 (74.19) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{59.30 (38.47)} & 2 & 138.52 (75.87) & 3 & 233.73 (39.89) & \cellcolor{green!20}2 & \cellcolor{green!20}177.35 (384.90) & 3 & 1194.11 (1403.01) & \textbf{1} & \textbf{1368.20 (250.10)} & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{62.50 (21.15)} & 2 & 87.44 (21.38) & \textbf{1} & \textbf{65.34 (21.07)} & 3 & 199.28 (45.12) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & 2 & 129.60 (73.04) & 3 & 191.77 (38.43) & \cellcolor{green!20}2 & \cellcolor{green!20}134.99 (522.74) & 3 & 1041.55 (230.02) & \textbf{1} & \textbf{1396.16 (189.09)} & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{48.69 (10.31)} & 3 & 65.20 (18.86) & 2 & 54.19 (10.26) & 4 & 158.05 (37.81) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{35.29 (17.13)} & 2 & 114.69 (48.99) & 3 & 172.70 (46.58) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{605.42 (1213.79)} & 3 & 1014.62 (255.48) & 2 & 1266.23 (184.09) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{44.15 (8.53)} & 3 & 52.53 (9.96) & 2 & 48.74 (9.81) & 4 & 132.03 (25.97) \\ \hline
\multirow{5}{*}{\textsc{SQLite}} & $S_1$ & 2 & 73.52 (20.40) & \textbf{1} & \textbf{68.63 (16.67)} & \cellcolor{red!20}3 & \cellcolor{red!20}65.45 (19.46) & 2 & 105.75 (83.62) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{74.67 (20.68)} & \textbf{1} & \textbf{76.22 (21.29)} & 3 & 82.77 (20.99) & \textbf{1} & \textbf{65.16 (12.06)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{62.32 (11.64)} & 2 & 70.76 (20.26) \\
 & $S_2$ & 2 & 76.41 (16.66) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{70.36 (14.36)} & \textbf{1} & \textbf{70.52 (24.47)} & 3 & 161.86 (135.45) & 2 & 95.26 (36.34) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{89.04 (34.14)} & 3 & 86.76 (20.84) & \textbf{1} & \textbf{69.64 (10.76)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{64.04 (13.07)} & 2 & 75.59 (24.63) \\
 & $S_3$ & \textbf{1} & \textbf{71.63 (11.58)} & \cellcolor{red!20}2 & \cellcolor{red!20}67.30 (12.50) & \textbf{1} & \textbf{69.51 (14.85)} & 3 & 103.75 (29.66) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{76.20 (21.41)} & 2 & 84.61 (35.20) & 3 & 87.65 (24.29) & \textbf{1} & \textbf{69.77 (13.75)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{64.25 (11.83)} & 2 & 70.77 (18.66) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & 2 & 69.71 (10.60) & 2 & 70.93 (11.85) & 2 & 82.25 (23.16) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{68.94 (13.83)} & 2 & 82.27 (27.41) & 3 & 86.47 (20.30) & 2 & 69.29 (9.25) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{62.19 (11.78)} & 2 & 70.01 (16.80) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & 2 & 69.41 (10.96) & 2 & 71.51 (14.27) & 2 & 76.06 (16.27) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{68.03 (10.38)} & 3 & 80.61 (23.78) & 3 & 84.43 (12.41) & 2 & 70.42 (9.55) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{63.59 (12.77)} & 2 & 71.19 (13.68) \\ \hline
\multirow{5}{*}{\textsc{x264}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.21 (4.35)} & 3 & 13.65 (14.17) & 2 & 15.17 (5.23) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.43 (3.40)} & \textbf{1} & \textbf{10.90 (2.21)} & \textbf{1} & \textbf{11.58 (2.30)} & 2 & 10.40 (2.15) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.18 (2.78)} & 3 & 11.19 (2.06) & 4 & 12.22 (5.95) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.72 (1.52)} & 3 & 8.44 (24.28) & 2 & 8.68 (2.80) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.51 (0.98)} & 2 & 8.11 (1.06) & 3 & 8.74 (1.21) & \textbf{1} & \textbf{6.57 (1.67)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.42 (1.20)} & 3 & 8.53 (0.86) & 2 & 6.82 (1.28) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.57 (1.52)} & 2 & 5.06 (48.28) & 2 & 6.73 (57.61) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.84 (0.52)} & 2 & 7.57 (0.81) & 3 & 7.91 (0.80) & \textbf{1} & \textbf{5.01 (1.42)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.95 (0.85)} & 3 & 7.45 (0.85) & 2 & 5.59 (0.64) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.30 (1.17)} & 2 & 4.04 (45.08) & 2 & 4.86 (39.30) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.52)} & 2 & 7.27 (0.45) & 3 & 7.44 (0.37) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.52 (1.33)} & 2 & 4.04 (0.86) & 4 & 6.61 (0.73) & 3 & 4.53 (0.67) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.96 (0.79)} & 2 & 3.80 (28.85) & 2 & 3.98 (3.19) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.10 (1.04)} & 2 & 7.12 (0.67) & 3 & 7.19 (0.46) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.54 (1.04)} & 2 & 2.98 (0.77) & 4 & 6.26 (0.58) & 3 & 3.55 (0.53) \\ \hline
\multirow{5}{*}{\textsc{Dune}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{9.37 (1.15)} & 3 & 13.64 (1.55) & 2 & 12.26 (0.86) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.21 (0.88)} & 2 & 13.01 (1.78) & 3 & 13.76 (5.73) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{9.04 (1.13)} & \textbf{1} & \textbf{9.27 (0.56)} & 2 & 10.12 (0.71) & \textbf{1} & \textbf{9.29 (0.65)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & 2 & 8.72 (2.48) & 3 & 9.66 (1.10) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.13 (0.57)} & 2 & 12.94 (1.04) & 3 & 27.72 (8.04) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.25 (0.42)} & 3 & 7.27 (0.40) & 4 & 8.39 (0.26) & 2 & 6.62 (0.36) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & 2 & 7.87 (1.49) & 3 & 8.77 (1.21) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.09 (0.54)} & 2 & 13.10 (0.50) & 3 & 29.45 (5.73) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.48 (0.42)} & 3 & 6.63 (0.33) & 4 & 8.07 (0.24) & 2 & 5.79 (0.24) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & 2 & 7.22 (0.99) & 3 & 8.58 (0.97) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.04 (0.43)} & 2 & 13.15 (0.47) & 3 & 29.21 (5.15) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.06 (0.32)} & 3 & 5.97 (0.45) & 4 & 7.85 (0.26) & 2 & 5.26 (0.19) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & 3 & 9.57 (2.40) & 2 & 9.36 (0.92) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.93 (0.48)} & 2 & 13.15 (0.61) & 3 & 29.14 (3.85) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.69 (0.35)} & 3 & 5.68 (0.35) & 4 & 7.66 (0.17) & 2 & 4.90 (0.23) \\ \hline
\multirow{5}{*}{\textsc{HIPA$^{cc}$}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.50 (1.42)} & 2 & 10.21 (0.86) & 2 & 10.19 (0.66) & \cellcolor{green!20}2 & \cellcolor{green!20}12.70 (1.22) & 3 & 20.95 (699.46) & \textbf{1} & \textbf{23.50 (2.17)} & 2 & 12.03 (0.93) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{11.08 (0.66)} & \textbf{1} & \textbf{11.19 (0.60)} & 3 & 14.24 (0.61) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & 2 & 7.41 (1.03) & 3 & 7.87 (0.86) & \cellcolor{green!20}3 & \cellcolor{green!20}11.64 (0.35) & \textbf{1} & \textbf{19.70 (0.89)} & 2 & 21.82 (0.68) & \textbf{1} & \textbf{8.47 (1.10)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.46 (0.70)} & 2 & 9.88 (0.37) & 3 & 10.48 (0.63) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & 2 & 6.14 (0.96) & 2 & 6.55 (0.68) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.43 (0.34)} & 2 & 19.34 (0.88) & 3 & 21.82 (0.42) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.62 (0.80)} & \textbf{1} & \textbf{6.69 (0.51)} & 3 & 9.41 (0.33) & 2 & 8.21 (0.47) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & 2 & 4.31 (0.77) & 3 & 5.07 (0.74) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.13 (0.25)} & 2 & 18.94 (0.58) & 3 & 21.75 (0.81) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.42 (0.22)} & 2 & 4.47 (0.32) & 4 & 8.81 (0.20) & 3 & 5.37 (0.24) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & 2 & 3.04 (0.81) & 3 & 3.86 (0.58) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{11.01 (0.15)} & 2 & 18.79 (0.35) & 3 & 21.88 (0.76) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.69 (0.15)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.69 (0.13)} & 3 & 8.30 (0.20) & 2 & 3.10 (0.13) \\ \hline
\multirow{5}{*}{\textsc{HSMGP}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & 2 & 7.01 (1.39) & 2 & 8.63 (1.77) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.72 (0.80)} & 2 & 55.90 (20.70) & 3 & 80.26 (38.86) & 3 & 21.65 (2.31) & 2 & 16.63 (2.10) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{14.63 (1.92)} & 4 & 25.42 (5.90) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & 3 & 4.85 (4.52) & 2 & 5.61 (1.17) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.35 (0.47)} & 2 & 51.49 (11.94) & 3 & 81.46 (17.14) & 3 & 15.59 (1.41) & 2 & 11.46 (1.78) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{10.59 (0.88)} & 4 & 18.59 (1.67) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & 2 & 3.60 (0.69) & 3 & 3.87 (0.75) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.14 (0.35)} & 2 & 51.65 (8.15) & 3 & 80.54 (19.98) & 2 & 11.35 (0.63) & \textbf{1} & \textbf{7.58 (0.67)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.52 (0.46)} & 3 & 12.10 (0.67) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & 2 & 3.57 (0.95) & 2 & 3.91 (0.73) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.16 (0.17)} & 2 & 49.96 (10.24) & 3 & 66.32 (36.72) & 3 & 10.13 (0.57) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.88 (0.61)} & 2 & 7.10 (0.38) & 4 & 10.47 (0.65) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & 2 & 3.02 (1.31) & 2 & 3.58 (0.78) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.15 (0.20)} & 2 & 49.18 (3.13) & 3 & 85.14 (39.24) & 4 & 7.46 (0.46) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.15 (0.28)} & 2 & 6.11 (0.26) & 3 & 7.04 (0.28) \\ \hline
\multirow{5}{*}{\textsc{Lrzip}} & $S_1$ & \textbf{1} & \textbf{31.88 (10.96)} & \cellcolor{red!20}2 & \cellcolor{red!20}31.78 (29.81) & 3 & 70.36 (28.67) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{117.37 (24.65)} & 2 & 363.17 (114.48) & 3 & 475.86 (188.56) & 2 & 17.95 (10.85) & 3 & 21.71 (7.45) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{16.71 (4.27)} & 4 & 76.46 (23.85) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & 2 & 46.26 (25.10) & 3 & 74.19 (33.01) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{109.11 (20.26)} & 2 & 315.54 (57.21) & 3 & 474.88 (196.54) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{9.09 (2.56)} & 2 & 10.18 (2.12) & \textbf{1} & \textbf{10.19 (1.79)} & 3 & 36.47 (12.40) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & 2 & 30.06 (17.51) & 3 & 59.65 (24.60) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{104.20 (17.55)} & 2 & 321.82 (49.06) & 3 & 360.11 (241.44) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.77 (2.09)} & \textbf{1} & \textbf{7.90 (1.27)} & 2 & 8.43 (0.69) & 3 & 26.46 (7.48) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & 2 & 31.16 (20.54) & 3 & 71.33 (22.86) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{103.74 (14.29)} & 2 & 325.19 (51.13) & 3 & 346.60 (131.69) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.38 (2.72)} & \textbf{1} & \textbf{6.51 (0.69)} & 2 & 7.59 (0.91) & 3 & 19.77 (2.80) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & 2 & 23.74 (4.27) & 3 & 58.48 (34.30) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{105.83 (7.06)} & 2 & 324.82 (32.57) & 3 & 457.93 (299.67) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.58 (0.97)} & 2 & 3.67 (1.31) & 2 & 6.17 (0.43) & 3 & 9.37 (1.21) \\ \hline
\multirow{5}{*}{\textsc{nginx}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & 2 & 24.02 (12.20) & 3 & 34.82 (21.61) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{22.02 (2.11)} & 3 & 576.17 (24.71) & 2 & 550.28 (66.10) & 3 & 14.44 (2.41) & 4 & 84.12 (150.39) & 2 & 6.78 (1.92) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.23 (1.21)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & 2 & 22.99 (9.15) & 3 & 28.21 (2.89) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{20.25 (1.60)} & 2 & 568.78 (17.19) & 2 & 564.04 (37.05) & 3 & 7.44 (3.14) & 4 & 11.09 (3.33) & 2 & 4.90 (0.44) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.17 (0.48)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & 2 & 23.32 (8.65) & 3 & 27.64 (5.37) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{19.66 (0.75)} & 2 & 567.70 (19.05) & 2 & 570.41 (23.98) & 2 & 4.81 (0.81) & 3 & 5.68 (1.43) & 2 & 4.56 (0.09) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.85 (0.43)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & 2 & 14.92 (9.09) & 3 & 24.84 (4.19) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{19.74 (0.82)} & 2 & 566.35 (18.53) & 2 & 566.60 (22.75) & 2 & 4.16 (1.01) & 4 & 4.87 (0.63) & 3 & 4.49 (0.05) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.59 (0.28)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & 2 & 6.11 (6.87) & 3 & 11.91 (11.63) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{19.17 (1.07)} & 2 & 565.62 (23.39) & 2 & 567.96 (18.51) & 2 & 3.33 (1.00) & 3 & 4.49 (0.56) & 3 & 4.44 (0.06) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.64 (0.30)} \\ \hline
\multirow{5}{*}{\textsc{VP8}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & 3 & 6.05 (1.14) & 2 & 8.31 (0.68) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.72 (0.84)} & 3 & 45.51 (7.20) & 2 & 44.69 (5.11) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.57 (0.70)} & 3 & 3.32 (0.79) & 3 & 5.99 (0.31) & 2 & 4.42 (0.46) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & 3 & 3.34 (1.09) & 2 & 3.56 (0.43) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.42 (0.44)} & 2 & 42.04 (3.29) & 2 & 42.06 (2.51) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.24 (0.24)} & 2 & 1.45 (0.16) & 3 & 5.25 (0.20) & 2 & 1.44 (0.21) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & 3 & 2.91 (0.32) & 2 & 2.66 (0.35) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.41 (0.34)} & 2 & 42.55 (2.55) & 3 & 44.06 (2.66) & 2 & 1.15 (0.12) & 2 & 1.16 (0.16) & 3 & 5.15 (0.15) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.11 (0.09)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & 3 & 2.48 (0.39) & 2 & 2.22 (0.33) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.35 (0.31)} & 2 & 41.90 (3.11) & 3 & 42.98 (2.47) & 3 & 1.07 (0.08) & 2 & 1.03 (0.11) & 4 & 5.07 (0.10) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.02 (0.05)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & 3 & 2.20 (0.33) & 2 & 1.66 (0.16) & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.41 (0.27)} & 2 & 42.79 (1.80) & 3 & 43.19 (2.36) & 3 & 0.94 (0.04) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.85 (0.03)} & 4 & 4.89 (0.09) & 2 & 0.88 (0.04) \\ \hline
\multicolumn{2}{c}{Average $r$} & 1.03 &  & 2.22 &  & 2.42 &  & 1.2 &  & 2.1 &  & 2.38 &  & 1.85 &  & 2 &  & 2.35 &  & 2.43 &   \\ 
\bottomrule
\end{tabular}
}
% \end{table*}

==> Tables/response_ensemble_DNN.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
\begin{tabular}{clllllll}
\toprule
\multirow{2}{*}{System} & \multicolumn{1}{c}{\multirow{2}{*}{Size}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{Bagging$_{HINN}$}} & \multicolumn{2}{c}{\texttt{AdaBoost$_{HINN}$}} \\ \cline{3-8}
 & \multicolumn{1}{c}{} & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) \\ \hline
\multirow{5}{*}{\textsc{Apache}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.86 (7.36)} & 3 & 24.64 (9.80) & 2 & 24.78 (6.66) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{12.89 (7.87)} & \textbf{1} & \textbf{14.84 (6.31)} & \textbf{1} & \textbf{15.61 (5.39)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & 2 & 11.20 (5.52) & 3 & 12.19 (10.08) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.87 (1.95)} & 3 & 9.17 (23.67) & 2 & 9.86 (2.32) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & 3 & 7.81 (24.03) & 2 & 8.90 (3.19) \\ \hline
\multirow{5}{*}{\textsc{BDB-C}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{83.60 (208.75)} & \textbf{1} & \textbf{158.49 (97.21)} & 2 & 239.27 (165.36) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.92 (17.91)} & 2 & 87.45 (64.92) & 3 & 175.89 (62.71) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.31 (7.52)} & 2 & 52.55 (22.07) & 3 & 100.26 (43.36) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.60 (4.50)} & 2 & 35.88 (17.56) & 3 & 77.71 (33.23) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & 2 & 31.49 (17.12) & 3 & 58.63 (19.41) \\ \hline
\multirow{5}{*}{\textsc{BDB-J}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.37 (4.74)} & 2 & 11.23 (6.65) & 2 & 14.06 (7.13) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & 3 & 5.24 (33.48) & 2 & 5.17 (3.19) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & 3 & 3.29 (1.29) & 2 & 3.75 (0.62) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & 3 & 2.93 (0.80) & 2 & 2.70 (0.59) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.40 (0.34)} & 3 & 2.48 (0.56) & 2 & 2.39 (0.38) \\ \hline
\multirow{5}{*}{\textsc{kanzi}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & 2 & 256.87 (151.84) & 3 & 410.20 (187.36) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{95.31 (51.34)} & 2 & 184.70 (53.30) & 3 & 285.91 (71.88) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{59.30 (38.47)} & 2 & 138.52 (75.87) & 3 & 233.73 (39.89) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & 2 & 129.60 (73.04) & 3 & 191.77 (38.43) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{35.29 (17.13)} & 2 & 114.69 (48.99) & 3 & 172.70 (46.58) \\ \hline
\multirow{5}{*}{\textsc{SQLite}} & $S_1$ & 2 & 73.52 (20.40) & \textbf{1} & \textbf{68.63 (16.67)} & \cellcolor{red!20}3 & \cellcolor{red!20}65.45 (19.46) \\
 & $S_2$ & 2 & 76.41 (16.66) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{70.36 (14.36)} & \textbf{1} & \textbf{70.52 (24.47)} \\
 & $S_3$ & \textbf{1} & \textbf{71.63 (11.58)} & \cellcolor{red!20}2 & \cellcolor{red!20}67.30 (12.50) & \textbf{1} & \textbf{69.51 (14.85)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & 2 & 69.71 (10.60) & 2 & 70.93 (11.85) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & 2 & 69.41 (10.96) & 2 & 71.51 (14.27) \\ \hline
\multirow{5}{*}{\textsc{x264}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.21 (4.35)} & 3 & 13.65 (14.17) & 2 & 15.17 (5.23) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.72 (1.52)} & 3 & 8.44 (24.28) & 2 & 8.68 (2.80) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.57 (1.52)} & 2 & 5.06 (48.28) & 2 & 6.73 (57.61) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.30 (1.17)} & 2 & 4.04 (45.08) & 2 & 4.86 (39.30) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.96 (0.79)} & 2 & 3.80 (28.85) & 2 & 3.98 (3.19) \\ \hline
\multirow{5}{*}{\textsc{Dune}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{9.37 (1.15)} & 3 & 13.64 (1.55) & 2 & 12.26 (0.86) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & 2 & 8.72 (2.48) & 3 & 9.66 (1.10) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & 2 & 7.87 (1.49) & 3 & 8.77 (1.21) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & 2 & 7.22 (0.99) & 3 & 8.58 (0.97) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & 3 & 9.57 (2.40) & 2 & 9.36 (0.92) \\ \hline
\multirow{5}{*}{\textsc{HIPA$^{cc}$}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.50 (1.42)} & 2 & 10.21 (0.86) & 2 & 10.19 (0.66) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & 2 & 7.41 (1.03) & 3 & 7.87 (0.86) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & 2 & 6.14 (0.96) & 2 & 6.55 (0.68) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & 2 & 4.31 (0.77) & 3 & 5.07 (0.74) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & 2 & 3.04 (0.81) & 3 & 3.86 (0.58) \\ \hline
\multirow{5}{*}{\textsc{HSMGP}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & 2 & 7.01 (1.39) & 2 & 8.63 (1.77) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & 3 & 4.85 (4.52) & 2 & 5.61 (1.17) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & 2 & 3.60 (0.69) & 3 & 3.87 (0.75) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & 2 & 3.57 (0.95) & 2 & 3.91 (0.73) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & 2 & 3.02 (1.31) & 2 & 3.58 (0.78) \\ \hline
\multirow{5}{*}{\textsc{Lrzip}} & $S_1$ & \textbf{1} & \textbf{31.88 (10.96)} & \cellcolor{red!20}2 & \cellcolor{red!20}31.78 (29.81) & 3 & 70.36 (28.67) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & 2 & 46.26 (25.10) & 3 & 74.19 (33.01) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & 2 & 30.06 (17.51) & 3 & 59.65 (24.60) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & 2 & 31.16 (20.54) & 3 & 71.33 (22.86) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & 2 & 23.74 (4.27) & 3 & 58.48 (34.30) \\ \hline
\multirow{5}{*}{\textsc{nginx}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & 2 & 24.02 (12.20) & 3 & 34.82 (21.61) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & 2 & 22.99 (9.15) & 3 & 28.21 (2.89) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & 2 & 23.32 (8.65) & 3 & 27.64 (5.37) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & 2 & 14.92 (9.09) & 3 & 24.84 (4.19) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & 2 & 6.11 (6.87) & 3 & 11.91 (11.63) \\ \hline
\multirow{5}{*}{\textsc{VP8}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & 3 & 6.05 (1.14) & 2 & 8.31 (0.68) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & 3 & 3.34 (1.09) & 2 & 3.56 (0.43) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & 3 & 2.91 (0.32) & 2 & 2.66 (0.35) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & 3 & 2.48 (0.39) & 2 & 2.22 (0.33) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & 3 & 2.20 (0.33) & 2 & 1.66 (0.16) \\ \hline
\multicolumn{2}{c}{Average $r$} & 1.03 &  & 2.22 &  & 2.42 & 
\\
\bottomrule
\end{tabular}
% \end{table}

==> Tables/response_time.tex <==
% \begin{table}[]
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabular}{ll}
\toprule
\textbf{Approach} & \textbf{Overhead (minutes)} \\ \hline

\texttt{DaL$_{LR}$} & \textcolor{black}{2$\times 10^{-4}$ to 0.32} \\
--- \Model~(\textit{adapting $d$}) & 1$\times 10^{-6}$ to 0.02 \\
--- \Model~(\textit{dividing}) & 9$\times 10^{-4}$ to 0.18 \\
--- \Model~(\textit{training}) & 3$\times 10^{-}4$ to 0.21 \\
--- \Model~(\textit{predicting}) & 4$\times 10^{-}5$ to 0.09 \\

\texttt{DaL$_{CART}$} & \textcolor{black}{1$\times 10^{-3}$ to 0.55} \\
--- \Model~(\textit{adapting $d$}) & 1$\times 10^{-6}$ to 0.02 \\
--- \Model~(\textit{dividing}) & 9$\times 10^{-4}$ to 0.18 \\
--- \Model~(\textit{training}) & 2$\times 10^{-4}$ to 0.31 \\
--- \Model~(\textit{predicting}) & 5$\times 10^{-4}$ to 0.10 \\

\Model & 4 to 56 \\
--- \Model~(\textit{adapting $d$}) & 1$\times 10^{-6}$ to 0.02 \\
--- \Model~(\textit{dividing}) & 9$\times 10^{-4}$ to 0.18 \\
--- \Model~(\textit{training}) & 3 to 53 \\
--- \Model~(\textit{predicting}) & 0.3 to 3 \\
\bottomrule
\end{tabular}
\end{subtable}
\hspace{0.6cm}
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabular}{ll}
\toprule
\textbf{Approach} & \textbf{Overhead (minutes)} \\ \hline~\vspace{0.1cm}
\texttt{SPLConqueror} & 4$\times 10^{-4}$ to 5$\times 10^{-3}$ \\~\vspace{0.12cm}
\texttt{AdaBoost$_{LR}$} & \textcolor{black}{5$\times 10^{-6}$ to 8$\times 10^{-3}$} \\~\vspace{0.12cm}
\texttt{RF} & \textcolor{black}{1$\times 10^{-4}$ to 8$\times 10^{-3}$} \\~\vspace{0.12cm}
\texttt{XGBoost} & \textcolor{black}{3$\times 10^{-4}$ to 8$\times 10^{-3}$} \\~\vspace{0.12cm}
\texttt{Adaboost$_{CART}$} & \textcolor{black}{5$\times 10^{-5}$ to 0.02} \\~\vspace{0.12cm}
\texttt{Bagging$_{LR}$} & \textcolor{black}{1$\times 10^{-3}$ to 0.02} \\~\vspace{0.12cm}
\texttt{DECART} & 0.07 to 0.5 \\~\vspace{0.12cm}
\texttt{Perf-AL} & 0.08 to 2.4 \\~\vspace{0.12cm}
\texttt{DeepPerf} & 3 to 48 \\~\vspace{0.12cm}
\texttt{HINNPerf} & 3 to 54 \\~\vspace{0.12cm}
\texttt{AdaBoost$_{HINN}$} & \textcolor{black}{2.28 to 92.51} \\
~\texttt{Bagging$_{HINN}$} & \textcolor{black}{2.43 to 92.63} \\





\bottomrule
\end{tabular}
\end{subtable}
% \end{table}


%   \begin{subtable}[t]{0.45\textwidth}
%     \centering
% \small
% \begin{tabular}{lll}
% \toprule
% \multicolumn{1}{c}{\textbf{ID}} & \multicolumn{1}{c}{\textbf{Data Item}} & \multicolumn{1}{c}{\textbf{RQ}} \\ \hline
% $I_{1}$ & Authors & N/A \\ \hline
% $I_{2}$ & Year & N/A \\ \hline
% $I_{3}$ & Title & N/A \\ \hline
% $I_{4}$ & Venue (conference or journal) & N/A \\ \hline
% $I_{5}$ & Data preprocessing methods & RQ1 \\ \hline
% $I_{6}$ & Data encoding sachems & RQ1 \\ \hline
% $I_{7}$ & Data sampling strategies & RQ1 \\ \hline
% $I_{8}$ & Sparsity handling mechanisms & RQ2 \\ \hline
% $I_{9}$ & Deep learning models & RQ2 \\ \hline
% $I_{10}$ & Reasons for model selection & RQ2 \\ \hline
% $I_{11}$ & Hyperparameter tuning optimizers & RQ2 \\ 
% \bottomrule
% \end{tabular}
%   \end{subtable}
%   \hspace{0.6cm}
%   \begin{subtable}[t]{0.45\textwidth}
%     \centering
% \small
% \begin{tabular}{lll}
% \toprule
% \multicolumn{1}{c}{\textbf{ID}} & \multicolumn{1}{c}{\textbf{Data Item}} & \multicolumn{1}{c}{\textbf{RQ}} \\ \hline
% $I_{12}$ & Training algorithms & RQ2 \\ \hline
% $I_{13}$ & Activation functions & RQ2 \\ \hline
% $I_{14}$ & Evaluation procedures & RQ3 \\ \hline
% $I_{15}$ & Accuracy metrics & RQ3 \\ \hline
% $I_{16}$ & Statistical test & RQ3 \\ \hline
% $I_{17}$ & Effect size measurement & RQ3 \\ \hline
% $I_{18}$ & Number of subject systems & RQ3 \\ \hline
% $I_{19}$ & Domain of subject systems & RQ3 \\ \hline
% $I_{20}$ & Application categories & RQ4 \\ \hline
% $I_{21}$ & Handling of dynamic environments & RQ4 \\ \hline
% $I_{22}$ & Availability of code and dataset & RQ4
% \\ \bottomrule
% \end{tabular}
%   \end{subtable}

==> Tables/response_vs_FSE.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
\begin{tabular}{clllll}
\toprule
\multirow{2}{*}{System} & \multicolumn{1}{c}{\multirow{2}{*}{Size}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{DaL-FSE}} \\ \cline{3-6}
 & \multicolumn{1}{c}{} & $r$ & Med (IQR) & $r$ & Med (IQR) \\ \hline
\multirow{5}{*}{\textsc{Apache}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.86 (7.36)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{21.86 (7.36)} \\
 & $S_2$ & \textbf{1} & \textbf{12.89 (7.87)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{11.87 (9.22)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.56 (1.92)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.87 (1.95)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.87 (1.95)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.78 (1.08)} \\ \hline
\multirow{5}{*}{\textsc{BDB-C}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{83.60 (208.75)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{83.60 (208.75)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{21.92 (17.91)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{21.92 (17.91)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.31 (7.52)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.31 (7.52)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.60 (4.50)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{3.60 (4.50)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.88 (1.24)} \\ \hline
\multirow{5}{*}{\textsc{BDB-J}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.37 (4.74)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.37 (4.74)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.83 (0.45)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.58 (0.26)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.45 (0.22)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.40 (0.34)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.40 (0.34)} \\ \hline
\multirow{5}{*}{\textsc{kanzi}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{196.15 (213.73)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{95.31 (51.34)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{95.31 (51.34)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{59.30 (38.47)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{59.30 (38.47)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{42.93 (18.75)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{35.29 (17.13)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{35.29 (17.13)} \\ \hline
\multirow{5}{*}{\textsc{SQLite}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{73.52 (20.40)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{73.52 (20.40)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{76.41 (16.66)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{76.41 (16.66)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{71.63 (11.58)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{71.63 (11.58)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{66.94 (10.61)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{64.20 (13.91)} \\ \hline
\multirow{5}{*}{\textsc{x264}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.21 (4.35)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{10.21 (4.35)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.72 (1.52)} & \textbf{1} & \textbf{2.74 (1.36)} \\
 & $S_3$ & 2 & 1.57 (1.52) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.56 (0.70)} \\
 & $S_4$ & 2 & 1.30 (1.17) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.00 (0.56)} \\
 & $S_5$ & 2 & 0.96 (0.79) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.60 (0.36)} \\ \hline
\multirow{5}{*}{\textsc{Dune}} & $S_1$ & \textbf{1} & \textbf{9.37 (1.15)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{9.19 (0.89)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.95 (0.54)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.81 (0.48)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.23 (0.35)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{3.98 (0.19)} \\ \hline
\multirow{5}{*}{\textsc{HIPA$^{cc}$}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{7.50 (1.42)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.50 (1.42)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.48 (0.38)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{3.43 (0.34)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.60 (0.15)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.11 (0.08)} \\ \hline
\multirow{5}{*}{\textsc{HSMGP}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.14 (1.44)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.06 (0.19)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.42 (0.13)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.33 (0.08)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.19 (0.08)} \\ \hline
\multirow{5}{*}{\textsc{Lrzip}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{31.88 (10.96)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{31.88 (10.96)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{10.51 (4.39)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.04 (2.37)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{5.95 (0.99)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.03 (0.26)} \\ \hline
\multirow{5}{*}{\textsc{nginx}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{4.11 (1.45)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.60 (1.14)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.14 (0.40)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.99 (0.47)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.98 (0.21)} \\ \hline
\multirow{5}{*}{\textsc{VP8}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.56 (0.18)} \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.15 (0.05)} \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.08 (0.04)} \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.98 (0.05)} \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.90 (0.06)} \\ \hline
\multicolumn{2}{c}{Average $r$} & 1.05 &  & 1 & 
\\ \bottomrule
\end{tabular}
% \end{table}

==> Tables/response_vs_STOA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t!]
% \footnotesize
% \setlength{\tabcolsep}{1.2mm}
% \renewcommand\arraystretch{1.3}
\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{p{0.9cm}lp{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l|p{0.1cm}l} \toprule
\multirow{2}{*}{System} & \multicolumn{1}{c}{\multirow{2}{*}{Size}} & \multicolumn{2}{c}{\texttt{DaL}} & \multicolumn{2}{c}{\texttt{HINNPerf}} & \multicolumn{2}{c}{\texttt{DeepPerf}} & \multicolumn{2}{c}{\texttt{Perf-AL}} & \multicolumn{2}{c}{\texttt{DECART}} & \multicolumn{2}{c}{\texttt{SPLConqueror}} & \multicolumn{2}{c}{\texttt{IBMB}} & \multicolumn{2}{c}{\texttt{M5}} & \multicolumn{2}{c}{\texttt{PILOT}} & \multicolumn{2}{c}{\texttt{MOB}} \\ \cline{3-22}
 & \multicolumn{1}{c}{} & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) & $r$ & Med (IQR) \\ \hline
\multirow{5}{*}{\textsc{Apache}} & $S_1$ & 3 & 21.86 (7.36) & \cellcolor{red!20}3 & \cellcolor{red!20}19.44 (10.53) & 2 & 20.19 (6.34) & 8 & 33.57 (11.34) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{19.44 (6.48)} & 7 & 28.50 (11.14) & 4 & 25.09 (4.77) & 5 & 26.14 (4.51) & 7 & 28.50 (11.14) & 6 & 27.92 (8.28) \\
 & $S_2$ & 6 & 12.89 (7.87) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.93 (3.89)} & 2 & 9.79 (4.56) & 8 & 32.97 (6.24) & 3 & 9.77 (5.36) & 5 & 18.33 (2.96) & 6 & 25.62 (2.37) & 6 & 23.91 (3.24) & 4 & 17.61 (2.41) & 7 & 28.88 (3.88) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{6.56 (1.92)} & \textbf{1} & \textbf{7.01 (1.74)} & 2 & 7.98 (1.91) & 7 & 31.73 (4.66) & 2 & 8.07 (1.05) & 3 & 16.16 (1.41) & 5 & 25.92 (2.57) & 4 & 23.53 (2.09) & 3 & 16.16 (1.41) & 6 & 30.11 (3.62) \\
 & $S_4$ & 2 & 6.87 (1.95) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.58 (1.04)} & 2 & 6.85 (1.60) & 7 & 30.67 (6.84) & 3 & 7.47 (0.72) & 4 & 16.12 (0.78) & 6 & 25.90 (3.04) & 5 & 23.14 (0.81) & 4 & 16.12 (0.78) & 7 & 30.30 (4.08) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.78 (1.08)} & \textbf{1} & \textbf{5.85 (0.99)} & 2 & 6.66 (1.61) & 7 & 30.45 (4.91) & 3 & 7.14 (0.89) & 4 & 16.12 (1.37) & 6 & 26.55 (2.26) & 5 & 23.04 (0.82) & 4 & 16.12 (1.37) & 7 & 30.79 (3.13) \\ \hline
\multirow{5}{*}{\textsc{BDB-C}} & $S_1$ & 4 & 83.60 (208.75) & 4 & 167.55 (144.47) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{43.66 (42.88)} & 3 & 82.38 (57.27) & 2 & 51.88 (45.91) & 7 & 772.44 (576.45) & 5 & 389.74 (289.18) & 6 & 505.90 (163.69) & 7 & 772.44 (579.59) & 6 & 539.31 (358.57) \\
 & $S_2$ & 3 & 21.92 (17.91) & 2 & 21.45 (13.61) & 2 & 18.17 (8.11) & 4 & 73.99 (22.51) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{13.37 (7.25)} & 6 & 526.69 (131.89) & 5 & 438.62 (165.58) & 6 & 541.59 (179.45) & 6 & 526.69 (131.89) & 7 & 626.96 (187.51) \\
 & $S_3$ & 2 & 8.31 (7.52) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{6.50 (9.20)} & 3 & 12.47 (4.08) & 3 & 69.74 (4.33) & \textbf{1} & \textbf{7.56 (5.07)} & 5 & 465.51 (88.42) & 4 & 437.64 (109.19) & 6 & 498.86 (126.41) & 5 & 465.51 (89.84) & 7 & 632.90 (112.44) \\
 & $S_4$ & \cellcolor{green!20}2 & \cellcolor{green!20}3.60 (4.50) & \textbf{1} & \textbf{4.86 (2.18)} & 2 & 9.06 (9.76) & 3 & 69.50 (2.49) & \textbf{1} & \textbf{5.17 (5.07)} & 5 & 438.47 (85.57) & 4 & 399.19 (152.10) & 6 & 503.49 (109.97) & 5 & 443.62 (86.20) & 7 & 594.25 (164.09) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.88 (1.24)} & 3 & 4.04 (1.24) & 4 & 7.08 (8.03) & 5 & 69.29 (0.69) & 2 & 3.54 (1.92) & 7 & 461.53 (85.82) & 6 & 418.43 (143.13) & 8 & 486.14 (76.71) & 7 & 457.33 (85.98) & 9 & 618.53 (147.33) \\ \hline
\multirow{5}{*}{\textsc{BDB-J}} & $S_1$ & 3 & 5.37 (4.74) & 2 & 3.58 (1.74) & 3 & 2.98 (3.34) & 5 & 37.45 (2.45) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{2.36 (0.75)} & 5 & 43.23 (5.84) & 4 & 33.26 (3.52) & 4 & 33.71 (7.73) & 5 & 43.23 (6.80) & 6 & 51.89 (16.34) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.83 (0.45)} & \textbf{1} & \textbf{1.96 (0.36)} & 2 & 1.91 (0.68) & 5 & 37.90 (1.67) & \textbf{1} & \textbf{1.84 (0.17)} & 5 & 38.30 (5.35) & 4 & 32.86 (3.31) & 3 & 32.51 (5.51) & 5 & 38.35 (6.13) & 6 & 49.16 (10.89) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.58 (0.26)} & 2 & 1.75 (0.41) & 3 & 2.01 (1.10) & 6 & 37.19 (1.70) & \textbf{1} & \textbf{1.64 (0.24)} & 7 & 38.16 (3.88) & 4 & 32.04 (1.20) & 5 & 32.27 (3.41) & 7 & 38.20 (3.75) & 8 & 49.72 (5.45) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.45 (0.22)} & 2 & 1.52 (0.24) & 3 & 1.70 (0.37) & 6 & 37.74 (2.59) & \textbf{1} & \textbf{1.47 (0.12)} & 6 & 36.88 (2.95) & 4 & 31.83 (2.75) & 5 & 31.73 (4.46) & 6 & 37.00 (3.58) & 7 & 50.87 (6.77) \\
 & $S_5$ & \textbf{1} & \textbf{1.40 (0.34)} & 2 & 1.48 (0.32) & 3 & 1.69 (0.48) & 6 & 35.76 (4.47) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.37 (0.26)} & 7 & 37.23 (3.13) & 4 & 32.07 (3.14) & 5 & 31.81 (4.87) & 7 & 37.14 (2.97) & 8 & 51.11 (5.46) \\ \hline
\multirow{5}{*}{\textsc{kanzi}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{196.15 (213.73)} & 2 & 262.27 (175.07) & \textbf{1} & \textbf{196.36 (122.61)} & 5 & 1434.70 (1328.18) & 2 & 276.50 (272.43) & 6 & 2528.40 (662.30) & 2 & 216.42 (270.56) & 3 & 718.11 (341.73) & 7 & 3106.10 (1285.5) & 4 & 898.25 (391.69) \\
 & $S_2$ & 2 & 95.31 (51.34) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{80.53 (51.36)} & 3 & 107.12 (43.75) & 7 & 961.11 (877.82) & 3 & 126.50 (142.62) & 8 & 1197.63 (349.62) & 4 & 243.08 (214.68) & 5 & 700.77 (211.53) & 8 & 1198.90 (354.37) & 6 & 970.59 (585.52) \\
 & $S_3$ & \cellcolor{green!20}2 & \cellcolor{green!20}59.30 (38.47) & \textbf{1} & \textbf{62.20 (14.07)} & 2 & 68.62 (30.41) & 5 & 280.93 (147.45) & 3 & 74.08 (32.14) & 7 & 1059.46 (166.51) & 4 & 208.36 (88.01) & 6 & 782.13 (180.76) & 7 & 1059.46 (166.90) & 7 & 1002.12 (392.28) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{42.93 (18.75)} & \textbf{1} & \textbf{46.48 (19.58)} & 2 & 62.65 (26.54) & 5 & 266.53 (179.59) & 3 & 67.83 (15.79) & 7 & 1030.40 (166.98) & 4 & 160.99 (57.60) & 6 & 762.99 (208.45) & 7 & 1030.62 (163.83) & 7 & 1028.27 (269.47) \\
 & $S_5$ & \textbf{1} & \textbf{35.29 (17.13)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{34.27 (11.87)} & 2 & 49.42 (9.99) & 4 & 169.12 (64.60) & 3 & 67.27 (17.95) & 7 & 1012.03 (261.66) & 5 & 211.48 (104.22) & 6 & 749.61 (119.62) & 7 & 1011.45 (264.24) & 7 & 942.95 (295.12) \\ \hline
\multirow{5}{*}{\textsc{SQLite}} & $S_1$ & \textbf{1} & \textbf{73.52 (20.40)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{70.76 (27.86)} & 2 & 79.49 (25.36) & 6 & 573.26 (340.38) & \textbf{1} & \textbf{74.14 (17.98)} & 5 & 157.09 (70.92) & 6 & 199.96 (242.69) & 3 & 101.24 (26.56) & 4 & 151.86 (65.00) & 2 & 87.23 (2.08) \\
 & $S_2$ & \textbf{1} & \textbf{76.41 (16.66)} & 2 & 76.69 (23.32) & 3 & 77.75 (22.47) & 6 & 386.74 (323.30) & \cellcolor{red!20}2 & \cellcolor{red!20}76.20 (22.74) & 4 & 84.41 (23.00) & 4 & 81.65 (21.46) & 5 & 115.69 (29.35) & 4 & 84.41 (23.67) & 3 & 86.26 (1.95) \\
 & $S_3$ & \textbf{1} & \textbf{71.63 (11.58)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{71.02 (17.30)} & \textbf{1} & \textbf{75.01 (15.58)} & 5 & 424.32 (311.00) & \textbf{1} & \textbf{74.16 (20.12)} & 2 & 75.72 (24.82) & 2 & 72.53 (21.01) & 4 & 116.19 (29.50) & 2 & 75.72 (24.83) & 3 & 85.79 (1.46) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{66.94 (10.61)} & 2 & 70.84 (10.38) & 3 & 72.45 (12.11) & 6 & 363.18 (415.63) & 2 & 71.57 (14.72) & 3 & 69.61 (13.23) & 2 & 68.25 (13.72) & 5 & 120.45 (23.67) & 3 & 69.61 (13.80) & 4 & 85.61 (1.13) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{64.20 (13.91)} & 2 & 70.15 (9.71) & 3 & 72.87 (8.86) & 6 & 212.19 (295.12) & 2 & 68.51 (8.54) & 2 & 67.78 (9.68) & 2 & 66.01 (10.76) & 5 & 122.04 (17.73) & 2 & 67.78 (9.68) & 4 & 85.43 (1.26) \\ \hline
\multirow{5}{*}{\textsc{x264}} & $S_1$ & 3 & 10.21 (4.35) & 2 & 8.44 (2.69) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{8.04 (3.06)} & 7 & 37.00 (9.43) & 2 & 9.27 (2.11) & 4 & 12.70 (4.19) & 5 & 32.14 (0.49) & 5 & 32.21 (0.36) & 4 & 12.70 (4.19) & 6 & 34.59 (3.08) \\
 & $S_2$ & \cellcolor{green!20}2 & \cellcolor{green!20}2.72 (1.52) & \textbf{1} & \textbf{2.77 (1.07)} & 2 & 3.17 (1.00) & 8 & 34.98 (7.81) & 3 & 6.29 (1.72) & 4 & 8.01 (1.19) & 6 & 32.06 (0.76) & 5 & 31.67 (0.26) & 4 & 7.98 (1.32) & 7 & 34.43 (2.82) \\
 & $S_3$ & 2 & 1.57 (1.52) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{1.37 (0.46)} & 2 & 2.23 (0.90) & 8 & 36.25 (7.73) & 3 & 4.57 (1.03) & 4 & 7.61 (0.81) & 6 & 32.06 (0.40) & 5 & 31.54 (0.13) & 4 & 7.61 (0.88) & 7 & 34.57 (2.06) \\
 & $S_4$ & 2 & 1.30 (1.17) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.81 (0.28)} & 3 & 1.74 (0.98) & 8 & 36.41 (6.47) & 4 & 3.66 (1.42) & 5 & 7.31 (0.49) & 7 & 32.10 (0.36) & 6 & 31.51 (0.16) & 5 & 7.34 (0.45) & 8 & 34.67 (1.64) \\
 & $S_5$ & 2 & 0.96 (0.79) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{0.58 (0.15)} & 3 & 1.44 (0.90) & 8 & 36.20 (3.75) & 4 & 2.15 (1.05) & 5 & 7.11 (0.60) & 7 & 32.04 (0.30) & 6 & 31.50 (0.11) & 5 & 7.11 (0.60) & 8 & 34.37 (1.63) \\ \hline
\multirow{5}{*}{\textsc{Dune}} & $S_1$ & 3 & 9.37 (1.15) & 2 & 7.98 (0.98) & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.86 (0.93)} & 8 & 55.73 (0.12) & 9 & \texttimes & 4 & 13.03 (1.74) & 6 & 20.42 (2.38) & 7 & 22.71 (0.85) & 4 & 13.12 (1.91) & 5 & 18.39 (0.70) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.54)} & 2 & 6.15 (0.40) & \textbf{1} & \textbf{6.01 (0.21)} & 7 & 55.72 (0.53) & 8 & \texttimes & 3 & 13.09 (1.02) & 5 & 22.39 (2.06) & 6 & 22.89 (0.97) & 3 & 13.09 (0.99) & 4 & 18.52 (0.58) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.81 (0.48)} & 2 & 5.48 (0.39) & 2 & 5.52 (0.34) & 6 & 55.53 (1.69) & 7 & \texttimes & 3 & 13.17 (0.57) & 5 & 22.91 (2.02) & 5 & 22.95 (0.85) & 3 & 13.18 (0.59) & 4 & 18.48 (0.59) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.23 (0.35)} & 2 & 5.12 (0.38) & 3 & 5.26 (0.31) & 8 & 54.58 (1.48) & 9 & \texttimes & 4 & 13.15 (0.61) & 7 & 24.04 (1.39) & 6 & 22.85 (0.82) & 4 & 13.16 (0.61) & 5 & 18.75 (0.64) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.98 (0.19)} & 2 & 4.98 (0.64) & 3 & 5.15 (0.34) & 8 & 34.53 (21.14) & 9 & \texttimes & 4 & 13.17 (0.55) & 7 & 23.86 (1.77) & 6 & 22.96 (0.78) & 4 & 13.19 (0.52) & 5 & 18.49 (0.47) \\ \hline
\multirow{5}{*}{\textsc{HIPA$^{cc}$}} & $S_1$ & \textbf{1} & \textbf{7.50 (1.42)} & \cellcolor{red!20}\textbf{1} & \cellcolor{red!20}\textbf{7.40 (1.05)} & 2 & 9.70 (1.28) & 7 & 31.99 (0.06) & 8 & \texttimes & 3 & 20.43 (1.64) & 5 & 26.18 (0.68) & 4 & 25.01 (0.19) & 3 & 20.57 (1.85) & 6 & 33.07 (2.31) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.48 (0.38)} & 2 & 4.53 (0.48) & 3 & 6.89 (1.44) & 7 & 31.98 (0.06) & 9 & \texttimes & 4 & 19.73 (0.89) & 6 & 26.12 (0.49) & 5 & 24.97 (0.07) & 4 & 19.76 (0.86) & 8 & 33.79 (1.24) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{3.43 (0.34)} & 2 & 3.67 (0.28) & 3 & 4.68 (0.90) & 7 & 31.99 (0.06) & 9 & \texttimes & 4 & 19.33 (0.70) & 6 & 26.00 (0.46) & 5 & 24.95 (0.05) & 4 & 19.32 (0.85) & 8 & 33.73 (0.87) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (0.15)} & 2 & 2.70 (0.18) & 3 & 3.58 (1.00) & 7 & 31.98 (0.06) & 9 & \texttimes & 4 & 18.99 (0.61) & 6 & 25.90 (0.32) & 5 & 24.92 (0.06) & 4 & 18.99 (0.60) & 8 & 33.66 (0.79) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.11 (0.08)} & 2 & 2.23 (0.23) & 3 & 2.82 (0.57) & 7 & 31.97 (0.14) & 9 & \texttimes & 4 & 18.79 (0.42) & 6 & 25.73 (0.22) & 5 & 24.91 (0.12) & 4 & 18.79 (0.35) & 8 & 33.58 (0.66) \\ \hline
\multirow{5}{*}{\textsc{HSMGP}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.14 (1.44)} & 2 & 5.03 (2.56) & 3 & 7.09 (3.04) & 8 & 66.70 (1294.05) & 9 & \texttimes & 4 & 56.76 (18.43) & 5 & 65.36 (30.25) & 6 & 95.18 (11.51) & 4 & 56.76 (18.02) & 7 & 124.61 (36.63) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.06 (0.19)} & 2 & 3.13 (0.49) & 3 & 3.69 (0.61) & 8 & 66.67 (0.11) & 9 & \texttimes & 4 & 50.74 (12.37) & 5 & 67.20 (15.34) & 6 & 89.54 (8.16) & 4 & 50.85 (10.53) & 7 & 121.43 (23.60) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.42 (0.13)} & 2 & 2.34 (0.38) & 2 & 2.28 (0.37) & 6 & 66.63 (0.18) & 7 & \texttimes & 3 & 51.10 (8.01) & 4 & 62.29 (11.54) & 5 & 84.97 (4.24) & 3 & 51.73 (8.30) & 6 & 119.16 (16.57) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.33 (0.08)} & 2 & 2.19 (0.23) & 3 & 2.23 (0.39) & 6 & 66.63 (0.14) & 9 & \texttimes & 4 & 49.45 (9.49) & 5 & 62.38 (9.96) & 7 & 84.76 (5.45) & 4 & 50.41 (8.05) & 8 & 117.78 (15.89) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.19 (0.08)} & 2 & 2.09 (0.25) & 3 & 1.94 (0.63) & 6 & 66.59 (0.20) & 9 & \texttimes & 4 & 49.57 (3.15) & 5 & 58.63 (4.99) & 7 & 83.34 (3.06) & 4 & 49.58 (3.25) & 8 & 118.10 (7.24) \\ \hline
\multirow{5}{*}{\textsc{Lrzip}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{31.88 (10.96)} & 3 & 41.97 (12.02) & 2 & 35.40 (16.59) & 4 & 58.45 (0.12) & 9 & \texttimes & 6 & 353.37 (126.02) & 5 & 198.33 (88.16) & 7 & 416.66 (119.43) & 6 & 369.45 (117.97) & 8 & 556.01 (110.73) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{10.51 (4.39)} & 3 & 24.10 (19.98) & 2 & 21.46 (4.53) & 4 & 58.46 (0.18) & 9 & \texttimes & 6 & 309.08 (60.71) & 5 & 144.88 (72.46) & 7 & 403.42 (63.75) & 6 & 315.26 (62.54) & 8 & 517.67 (80.56) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{8.04 (2.37)} & 3 & 23.71 (16.49) & 2 & 18.68 (3.20) & 4 & 58.44 (0.21) & 9 & \texttimes & 6 & 317.52 (47.97) & 5 & 152.06 (92.00) & 7 & 389.89 (44.37) & 6 & 319.07 (50.92) & 8 & 531.18 (104.18) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{5.95 (0.99)} & 3 & 19.82 (16.76) & 2 & 15.55 (1.71) & 4 & 58.48 (0.21) & 9 & \texttimes & 6 & 318.37 (54.99) & 5 & 151.04 (54.46) & 7 & 385.47 (29.42) & 6 & 325.49 (47.06) & 8 & 531.05 (73.06) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.03 (0.26)} & 3 & 10.39 (2.92) & 2 & 10.17 (0.91) & 4 & 58.39 (0.21) & 9 & \texttimes & 6 & 325.68 (31.40) & 5 & 150.17 (20.91) & 7 & 383.70 (27.71) & 6 & 325.68 (30.81) & 8 & 531.16 (36.15) \\ \hline
\multirow{5}{*}{\textsc{nginx}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{4.11 (1.45)} & 2 & 8.08 (2.89) & 3 & 8.76 (4.10) & 7 & 1553.44 (965.63) & 8 & \texttimes & 4 & 574.23 (25.74) & 6 & 1218.33 (58.83) & 5 & 1042.65 (46.12) & 4 & 574.23 (25.74) & 7 & 1406.58 (65.16) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.60 (1.14)} & 2 & 6.95 (1.74) & 2 & 6.15 (4.17) & 7 & 1637.60 (430.94) & 8 & \texttimes & 3 & 566.48 (20.63) & 5 & 1200.34 (76.00) & 4 & 1046.84 (41.65) & 3 & 568.39 (20.34) & 6 & 1379.87 (80.17) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{2.14 (0.40)} & 3 & 6.46 (1.41) & 2 & 4.42 (1.44) & 8 & 1692.49 (305.78) & 9 & \texttimes & 4 & 567.42 (18.59) & 6 & 1206.44 (53.10) & 5 & 1045.37 (32.55) & 4 & 569.35 (15.63) & 7 & 1379.17 (61.17) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.99 (0.47)} & 3 & 6.01 (1.68) & 2 & 4.09 (2.27) & 8 & 1784.76 (274.62) & 9 & \texttimes & 4 & 568.66 (19.43) & 6 & 1203.30 (54.38) & 5 & 1046.87 (29.85) & 4 & 571.25 (18.43) & 7 & 1376.25 (59.62) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.98 (0.21)} & 3 & 7.27 (2.31) & 2 & 3.17 (1.72) & 8 & 1579.37 (515.54) & 9 & \texttimes & 4 & 564.37 (24.70) & 6 & 1199.31 (52.15) & 5 & 1039.58 (28.93) & 4 & 564.62 (23.57) & 7 & 1367.38 (60.70) \\ \hline
\multirow{5}{*}{\textsc{VP8}} & $S_1$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.56 (0.18)} & \textbf{1} & \textbf{1.72 (0.25)} & 2 & 4.68 (3.27) & 4 & 60.05 (2.03) & 8 & \texttimes & 3 & 44.06 (4.85) & 6 & 92.98 (4.52) & 5 & 85.03 (4.01) & 3 & 44.06 (4.20) & 7 & 110.78 (6.00) \\
 & $S_2$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.15 (0.05)} & 2 & 1.27 (0.15) & 3 & 2.39 (1.21) & 5 & 60.04 (0.24) & 9 & \texttimes & 4 & 42.10 (3.17) & 7 & 91.46 (5.56) & 6 & 85.68 (4.11) & 4 & 42.36 (3.42) & 8 & 108.46 (6.09) \\
 & $S_3$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{1.08 (0.04)} & 2 & 1.25 (0.14) & 3 & 1.93 (0.72) & 5 & 60.02 (0.29) & 9 & \texttimes & 4 & 42.94 (2.82) & 7 & 91.76 (3.49) & 6 & 84.88 (2.66) & 4 & 43.02 (2.62) & 8 & 108.23 (5.29) \\
 & $S_4$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.98 (0.05)} & 2 & 1.15 (0.11) & 3 & 1.54 (0.40) & 5 & 59.99 (0.27) & 9 & \texttimes & 4 & 42.05 (3.59) & 7 & 91.99 (3.14) & 6 & 84.78 (1.95) & 4 & 41.99 (3.12) & 8 & 108.47 (4.25) \\
 & $S_5$ & \cellcolor{green!20}\textbf{1} & \cellcolor{green!20}\textbf{0.90 (0.06)} & 2 & 1.12 (0.11) & 3 & 1.45 (0.23) & 5 & 59.95 (0.68) & 9 & \texttimes & 4 & 42.87 (2.39) & 7 & 92.21 (3.02) & 6 & 84.53 (2.44) & 4 & 42.66 (2.11) & 8 & 108.43 (3.71) \\ \hline
\multicolumn{2}{c}{Average $r$} & 1.47 &  & 1.88 &  & 2.37 &  & 6.1 &  & 5.38 &  & 4.67 &  & 5.13 &  & 5.45 &  & 4.65 &  & 6.62 & 
\\
\bottomrule
\end{tabular}
}
% \end{table*}


==> Tables/vs-STOA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \footnotesize
% \renewcommand\arraystretch{1.3}
%{p{0.7cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}}
\begin{tabular}{llllllllll}
\toprule
&
  Model &
  \textsc{Apache} &
  \textsc{BDB-C} &
  \textsc{BDB-J} &
  \textsc{x264} &
  \textsc{HSMGP} &
  \textsc{HIPA$^{cc}$} &
  \textsc{VP8} &
  \textsc{Lrzip} \\ \hline
 &
  \texttt{DeepPerf} &
  20.19(6.34) &
  75.98(70.55) &
  2.98(3.34) &
  8.39(4.77) &
  7.09(3.04) &
  9.70(1.28) &
  4.68(3.27) &
  35.40(16.59) \\
 &
  \texttt{\texttt{DECART}} &
  19.44(6.48) &
  \textbf{51.88(45.91)} &
  \textbf{2.36(0.75)} &
  9.27(2.11) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  33.57(11.34) &
  82.38(57.27) &
  37.45(2.45) &
  37.00(9.43) &
  66.70(1294.05) &
  31.99(0.06) &
  60.05(2.03) &
  58.45(0.12) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  \textbf{14.44(0)} &
  86.85(0) &
  12.29(0) &
  \textbf{7.01(0)} &
  15.04(0) &
  16.68(0) &
  \textbf{29.39(0)} &
  123.7(0) \\
\multirow{-5}{*}{Size 1} &
  \Model &
  21.02(6.64) &
  74.26(67.75) &
  3.14(2.90) &
  8.23(3.05) &
  \cellcolor{green!10}\textbf{4.66(1.32)} &
  \cellcolor{green!10}\textbf{9.07(1.18)} &
  \cellcolor{green!10}\textbf{1.59(0.36)} &
  \cellcolor{green!10}\textbf{26.40(6.94)} \\ \hline
 &
  \texttt{DeepPerf} &
  9.79(4.56) &
  17.58(8.01) &
  1.91(0.68) &
  3.17(1.00) &
  3.69(0.61) &
  6.89(1.44) &
  2.39(1.21) &
  21.46(4.53) \\
 &
  \texttt{\texttt{DECART}} &
  \textbf{9.77(5.36)} &
  \textbf{13.37(7.25)} &
  \textbf{1.84(0.17)} &
  6.29(1.72) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  32.97(6.24) &
  73.99(22.51) &
  37.90(1.67) &
  34.98(7.81) &
  66.67(0.11) &
  31.98(0.06) &
  60.04(0.24) &
  58.46(0.18) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  13.88(0) &
  162.91(0) &
  24.85(0) &
  6.63(0) &
  22.63(0) &
  16.96(0) &
  35.34(0) &
  171.85(0) \\
\multirow{-5}{*}{Size 2} &
  \Model &
  9.82(5.39) &
  18.32(17.04) &
  1.90(0.37) &
  \cellcolor{green!10}\textbf{3.21(1.95)} &
  \cellcolor{green!10}\textbf{2.66(0.68)} &
  \cellcolor{green!10}\textbf{5.55(0.60)} &
  \cellcolor{green!10}\textbf{1.21(0.09)} &
  \cellcolor{green!10}\textbf{15.37(6.04)} \\ \hline
 &
  \texttt{DeepPerf} &
  7.98(1.91) &
  12.47(4.08) &
  2.01(1.10) &
  2.23(0.90) &
  2.28(0.37) &
  4.68(0.90) &
  1.93(0.72) &
  18.68(3.20) \\
 &
  \texttt{\texttt{DECART}} &
  8.07(1.05) &
  7.56(5.07) &
  1.64(0.24) &
  4.57(1.03) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  31.73(4.66) &
  69.74(4.33) &
  37.19(1.70) &
  36.25(7.73) &
  66.63(0.18) &
  31.99(0.06) &
  60.02(0.29) &
  58.44(0.21) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  13.99(0) &
  193.89(0) &
  25.88(0) &
  6.31(0) &
  32.46(0) &
  17.18(0) &
  36.26(0) &
  177.61(0) \\
\multirow{-5}{*}{Size 3} &
  \Model &
  \cellcolor{green!10}\textbf{7.17(2.67)} &
  \cellcolor{green!10}\textbf{5.74(6.84)} &
  \cellcolor{green!10}\textbf{1.61(0.31)} &
  \cellcolor{green!10}\textbf{1.66(0.57)} &
  \cellcolor{green!10}\textbf{1.56(0.20)} &
  \cellcolor{green!10}\textbf{4.39(0.41)} &
  \cellcolor{green!10}\textbf{1.12(0.08)} &
  \cellcolor{green!10}\textbf{11.83(4.53)} \\ \hline
 &
  \texttt{DeepPerf} &
  6.85(1.60) &
  9.06(9.76) &
  1.70(0.37) &
  1.74(0.98) &
  2.23(0.39) &
  3.58(1.00) &
  1.54(0.40) &
  15.55(1.71) \\
 &
  \texttt{\texttt{DECART}} &
  7.47(0.72) &
  5.17(5.07) &
  \textbf{1.47(0.12)} &
  3.66(1.42) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  30.67(6.84) &
  69.50(2.49) &
  37.74(2.59) &
  36.41(6.47) &
  66.63(0.14) &
  31.98(0.06) &
  59.99(0.27) &
  58.48(0.21) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  13.84(0) &
  231.68(0) &
  29.01(0) &
  6.32(0) &
  33.73(0) &
  17.42(0) &
  37.14(0) &
  236.48(0) \\
\multirow{-5}{*}{Size 4} &
  \Model &
  \cellcolor{green!10}\textbf{6.59(1.77)} &
  \cellcolor{green!10}\textbf{3.68(2.78)} &
  1.61(0.29) &
  \cellcolor{green!10}\textbf{1.13(0.63)} &
  \cellcolor{green!10}\textbf{1.49(0.15)} &
  \cellcolor{green!10}\textbf{3.22(0.35)} &
  \cellcolor{green!10}\textbf{1.10(0.06)} &
  \cellcolor{green!10}\textbf{10.10(3.23)} \\ \hline
 &
  \texttt{DeepPerf} &
  6.66(1.61) &
  7.08(8.03) &
  1.69(0.48) &
  1.44(0.90) &
  1.94(0.68) &
  2.82(0.57) &
  1.45(0.23) &
  10.17(0.91) \\
 &
  \texttt{\texttt{DECART}} &
  7.14(0.89) &
  3.54(1.92) &
  \textbf{1.37(0.26)} &
  2.15(1.05) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  30.45(4.91) &
  69.29(0.69) &
  35.76(4.47) &
  36.20(3.75) &
  66.59(0.20) &
  31.97(0.14) &
  59.95(0.68) &
  58.39(0.21) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  14.06(0) &
  296.68(0) &
  29.87(0) &
  6.36(0) &
  35.86(0) &
  17.69(0) &
  36.21(0) &
  208.08(0) \\
\multirow{-5}{*}{Size 5} &
  \Model &
  \cellcolor{green!10}\textbf{5.96(2.07)} &
  \cellcolor{green!10}\textbf{2.15(1.52)} &
  1.46(0.26) &
  \cellcolor{green!10}\textbf{0.79(0.33)} &
  \cellcolor{green!10}\textbf{1.16(0.08)} &
  \cellcolor{green!10}\textbf{2.39(0.22)} &
  \cellcolor{green!10}\textbf{1.07(0.05)} &
  \cellcolor{green!10}\textbf{6.60(1.34)} \\
\bottomrule
\end{tabular}
% \end{table*}


==> Tables/vsDeepPerf.tex <==
% \begin{table*}[]
% \footnotesize
% \renewcommand\arraystretch{1.5}
% \caption{The median (IQR) of DeepPerf and \Model for all the subject sysmtems. 
% The \colorbox{red!10}{\textbf{cells}} mean DeepPerf is significantly better, and the \colorbox{green!10}{\textbf{cells}} mean \Model is significantly better.}
\resizebox{\textwidth}{!}{ % resize the table
\begin{tabular}{p{0.75cm}llp{0.2cm}llp{0.2cm}llp{0.2cm}llp{0.2cm}llp{0.2cm}}
\toprule
\multirow{2}{}{Subject system} &
  \multicolumn{3}{c}{Size 1} &
  \multicolumn{3}{c}{Size 2} &
  \multicolumn{3}{c}{Size 3} &
  \multicolumn{3}{c}{Size 4} &
  \multicolumn{3}{c}{Size 5} \\ \cline{2-16} 
 &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ \\ \hline
\textsc{Apache} &
  \multicolumn{1}{l}{20.19(6.34)} &
  \multicolumn{1}{l}{21.02(6.64)} &
  N &
  \multicolumn{1}{l}{9.79(4.56)} &
  \multicolumn{1}{l}{9.82(5.39)} &
  S &
  \multicolumn{1}{l}{7.98(1.91)} &
  \multicolumn{1}{l}{7.17(2.67)} &
  S &
  \multicolumn{1}{l}{6.85(1.60)} &
  \multicolumn{1}{l}{6.59(1.77)} &
  N &
  \multicolumn{1}{l}{6.66(1.61)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.96(2.07)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} \\ \hline
\textsc{BDB-C} &
  \multicolumn{1}{l}{75.98(70.55)} &
  \multicolumn{1}{l}{74.26(67.75)} &
  N &
  \multicolumn{1}{l}{17.58(8.01)} &
  \multicolumn{1}{l}{18.32(17.04)} &
  N &
  \multicolumn{1}{l}{12.47(4.08)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.74(6.84)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{9.06(9.76)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{3.68(2.78)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{7.08(8.03)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{2.15(1.52)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{BDB-J} &
  \multicolumn{1}{l}{2.98(3.34)} &
  \multicolumn{1}{l}{3.14(2.90)} &
  N &
  \multicolumn{1}{l}{1.91(0.68)} &
  \multicolumn{1}{l}{1.90(0.37)} &
  N &
  \multicolumn{1}{l}{2.01(1.10)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.61(0.31)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{1.70(0.37)} &
  \multicolumn{1}{l}{1.61(0.29)} &
  S &
  \multicolumn{1}{l}{1.69(0.48)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.46(0.26)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{x264} &
  \multicolumn{1}{l}{8.39(4.77)} &
  \multicolumn{1}{l}{8.23(3.05)} &
  N &
  \multicolumn{1}{l}{3.17(1.00)} &
  \multicolumn{1}{l}{3.21(1.95)} &
  N &
  \multicolumn{1}{l}{2.23(0.90)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.66(0.57)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{1.74(0.98)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.13(0.63)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{1.44(0.90)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{0.79(0.33)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{HSMGP} &
  \multicolumn{1}{l}{7.09(3.04)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{4.66(1.32)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{3.69(0.61)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{2.66(0.68)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{2.28(0.37)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.56(0.20)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{2.23(0.39)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.49(0.15)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
   \\ \hline
\textsc{HIPA$^{cc}$} &
  \multicolumn{1}{l}{9.70(1.28)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{9.07(1.18)}} &
  \cellcolor{green!10}\textbf{S$^\dagger$} &
  \multicolumn{1}{l}{6.89(1.44)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.55(0.60)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{4.68(0.90)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{4.39(0.41)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{3.58(1.00)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{3.22(0.35)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
   \\ \hline
\textsc{VP8} &
  \multicolumn{1}{l}{31.93(23.25)} &
  \multicolumn{1}{l}{29.73(20.29)} &
  N &
  \multicolumn{1}{l}{13.08(10.99)} &
  \multicolumn{1}{l}{9.70(11.92)} &
  S &
  \multicolumn{1}{l}{10.00(5.25)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.43(3.36)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{4.44(1.08)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{3.78(1.83)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{6.28(4.91)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{2.80(1.20)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{Lrzip} &
  \multicolumn{1}{l}{770.98(841.54)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{71.09(16.18)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{127.86(94.46)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{76.24(27.57)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{116.85(101)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{73.37(28.9)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{70.76(64.05)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{54.66(24.5)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{56.16(21.10)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{45.13(20.0)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} \\ \bottomrule
\end{tabular}
}
% \label{tb:vsDeepperf}
% \end{table*}



==> abstract.tex <==
\begin{abstract}


Predicting the performance of highly configurable software systems is the foundation for performance testing and quality assurance. To that end, recent work has been relying on machine/deep learning to model software performance. However, a crucial yet unaddressed challenge is how to cater for the sparsity inherited from the configuration landscape: the influence of configuration options (features) and the distribution of data samples are highly sparse. 

In this paper, we propose an approach based on the concept of ``divide-and-learn'', dubbed \Model. The basic idea is that, to handle sample sparsity, we divide the samples from the configuration landscape into distant divisions, for each of which we build a hierarchical and regularized Deep Neural Network as the local model to deal with the feature sparsity. A newly given configuration would then be assigned to the right model of division for the final prediction. 

Experiment results from eight real-world systems and five sets of training data reveal that, compared with the state-of-the-art approaches, \Model~performs no worse than the best counterpart on 33 out of 40 cases (within which 26 cases are significantly better) with up to $1.94\times$ improvement on accuracy; requires fewer samples to reach the same/better accuracy; and producing acceptable training overhead. Practically, \Model~also considerably improves different global models when using them as the underlying local models, which further strengthens its flexibility. To promote open science, all the data, code, and supplementary figures of this work can be accessed at our anonymous repository: \texttt{\textcolor{blue}{\url{https://github.com/Anoenymous/DaL}}}.

% \noindent\textbf{Background:} Modern software often provides a number of configurable options for users to meet their performance requirements. Due to the complex influence and interactions of the options, machine learning techniques have been applied to model the performance based on a set of measured performance data. Given the performance models are usually sparse, i.e. only a few options are actually influential, it is critical to adapt the ML models to fit the problem. However, many existing studies have ignored the sparsity problem, which could lead to a significant accuracy degradation. 

% \noindent\textbf{Aim:} This research aims at improving the accuracy of state-of-the-art performance prediction models by solving the sparsity problem.

% \noindent\textbf{Method:} We propose a 'Divide and Learn' framework, which splits the training data into subsets, learns each subset using a deep neural network separately, and then assigns the most suitable DNN to predict each testing sample. In that way, the sparsity in each subset is reduced and the DNN can learn the performance better.

% \noindent\textbf{Results:} Experiments on 8 real-world subject systems show that: (1) our DaL model outperforms the state-of-the-art deep learning model DeepPerf for all systems. (2) the framework can improve the accuracy of a number of ML models, and DNN is improved the most. (3) even considering the trade-off between accuracy and training time, our model is Pareto-optimal for half of the systems and (4) the best number of subsets to divide is two.

% \noindent\textbf{Conclusions:} This study contributes to the literature by addressing the often-ignored sparsity problem and improving the prediction accuracy of most of the ML models.

\end{abstract}

==> framework-knee.tex <==
\section{Divide-and-Learn: Divisible Learning for Configuration Performance}
\label{sec:framework}

% divide by similar performance, also some key option should also have similar values.

Drawing on our observations of the configuration data, we propose \Model~--- a framework of divisible learning that enables better prediction of the software configuration performance via ``divide-and-learn''. To mitigate the sample sparsity issue, the key idea of \Model~is that, since different divisions of configurations show drastically diverse characteristics, i.e., rather different performance values with distant values of key configuration options, we seek to independently learn a local model for each of those divisions that contain \textit{locally smooth} samples, thereby the learning can be more focused on the particular characteristics exhibited from the divisions and handle the feature sparsity. Yet, this requires us to formulate, on top of the original regression problem of predicting the performance value, a new classification problem without explicit labels. As such, we modify the original problem formulation (Equation~\ref{eq:prob}) as below: 
\begin{equation}
    \mathbfcal{D} = g(\mathbfcal{S}) 
\end{equation}
\begin{equation}
    \forall D_i \in \mathbfcal{D}\text{: } \mathcal{P} = f(D_i)\text{, } \mathcal{P}\in\mathbb{R}
\end{equation}
Overall, we aim to achieve three goals:

\begin{itemize}
    \item \textbf{Goal 1:} dividing the data samples into diverse yet more focused divisions $\mathbfcal{D}$ (building function $g$) and;
    \item \textbf{Goal 2:} training a dedicated local model for each division $D_i$ (building function $f$) while;
    \item \textbf{Goal 3:} assigning a newly coming configuration into the right model for prediction (using functions $g$ and $f$).
\end{itemize}



Figure~\ref{fig:structure} illustrates the overall architecture of \Model, in which there are three core phases, namely \textit{Dividing}, \textit{Training}, and \textit{Predicting}. A pseudo-code can also be found in Algorithm~\ref{alg:dal-code}. In particular, the options' interactions at the \textit{Division} are handled by CART and a parameter $d$, i.e., only the top options are considered in the process of dividing the data samples. In the \textit{Training}, the interaction between all options is considered by the local model. Yet, since the local model is only responsible for one division of the data, the full interactions are split, each of which is handled separately and independently. 




\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{Figures/overview.pdf}
  \caption{The architecture of \Model.}
  \label{fig:structure}
\end{figure}



% \begin{figure}[t!]
%   \centering
%   \include{Figures/landscape}
% %   \includegraphics[width=0.8\columnwidth]{Figures/landscape.tex}
%   \caption{A projected landscape of the performance objective Latency with respect to configuration options Splitters and Counters for Storm.}
%   \label{fig:landscape}
% \end{figure}

\subsection{Dividing}
\label{subsec:phase1_clustering}

The very first phase in \Model~is to appropriately divide the data into more focused divisions while doing so by considering both the configuration options and performance values. To that end, the key question we seek to address is: how to effectively cluster the performance data with similar sample characteristics (\textbf{Goal 1})? 



% To that end, we need to address two problems:

% \begin{itemize}
% \item How to efficiently filter the configuration options that do nothing but introduce noises?
% \item How to effectively cluster the performance data with similar sample characteristics? 
% \end{itemize}


% \subsubsection{Filtering Configuration Options with Mutual Information}

% It is important to rule out configuration options that do not make any contribution on the performance and doing so in an efficient manner especially when the data sample can be limited. Therefore, in \Model, we firstly calculate the Mutual Information (MI)~\cite{10.1093/biomet/70.1.163}, denoted as $I$, between an option and the performance. Fundamentally, MI measures the dependence between the two variables, i.e., in our context, this informs us about how much information we can gain about the performance when knowing the values of a particular configuration option. Formally, MI can be calculated as (assuming discretized variables):
% \begin{equation}
%     I(X,Y)=\sum_{x \in X}\sum_{y \in Y}p(x,y)\log({{p(x,y)} \over {p(x)p(y)}})
%     \label{eq:mi}
% \end{equation}
% whereby $x$ and $y$ denote a value for the configuration option and performance, receptively; $p$ refers to the probability function. We are particularly interested in finding those pairs that with $I=0$, which means the corresponding option can be removed, as it has no value at all in helping with the prediction. The computation of MI itself is rather cheap and hence serve as an efficient filter []. 
% %before we decide how to divide the data samples into more focused region.

% \subsubsection{Regression Tree as a Clustering Method}

\subsubsection{Modifying CART for Generating Divisions}

Indeed, for dividing the data samples, it makes sense to consider various unsupervised clustering algorithms, such as $k$-mean~\cite{macqueen1967some}, BIRCH~\cite{DBLP:conf/sigmod/ZhangRL96} or DBSCAN~\cite{DBLP:conf/kdd/EsterKSX96}. However, we found that they are ill-suited for our problem, because:

\begin{itemize}
    \item the distance metrics are highly system-dependent. For example, depending on the number of configuration options and whether they are binary/numeric options;
    \item it is difficult to combine the configuration options and performance value with appropriate discrimination; 
    %\item there is no tendency to ensure the likely prediction accuracy;
    \item and clustering algorithms are often non-interpretable.
\end{itemize}



As a result, in \Model, we extend Classification and Regression Tree (CART) as the clustering algorithm (lines 3-11 in Algorithm~\ref{alg:dal-code}) since (1) it is simple with interpretable/analyzable structure; (2) it ranks the important options as part of training (good for dealing with the feature sparsity issue), and (3) it does not suffer the issues above~\cite{DBLP:conf/kbse/SarkarGSAC15,DBLP:journals/ese/GuoYSASVCWY18,DBLP:journals/ase/NairMSA18,DBLP:conf/icse/Chen19b,DBLP:journals/tse/ChenB17,DBLP:journals/corr/abs-1801-02175,DBLP:conf/kbse/GuoCASW13}. In Section [], we will experimentally demonstrate that CART allows \Model~ to obtain much more superior results than the state-of-the-art clustering algorithms in dividing our configuration data.

As illustrated in Figure~\ref{fig:DT_example}, CART is originally a supervised and binary tree-structured model, which recursively splits some, if not all, configuration options and the corresponding data samples based on tuned thresholds. A split would result in two divisions, each of which can be further split. In this work, we at first train the CART on the available samples of configurations and performance values, during which we use the most common mean performance of all samples for each division $D_i$ as the prediction~\cite{DBLP:journals/ese/GuoYSASVCWY18,DBLP:conf/kbse/GuoCASW13}:
\begin{equation}
    \overline{y}_{D_i}={{1}\over{|D_i|}} {\sum_{y_j \in D_i}y_j}
    \label{eq:seg}
\end{equation}
in which $y_j$ is a performance value. For example, Figure~\ref{fig:DT_example} shows a projected example, in which the configuration that satisfies ``\texttt{rtQuality=true}'' and ``\texttt{threads=3}'' would lead to an inferred runtime of 112 seconds, which is calculated over all the 5 samples involved using Equation~\ref{eq:seg}.


\input{Tables/alg1}


\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{Figures/tree.pdf}
  \caption{Projection of CART for \textsc{VP8} showing the possible divisions with different colors under alternative depth $d$.}
  \label{fig:DT_example}
\end{figure}

By choosing/ranking options that serve as the splits and tuning their thresholds, in \Model, we seek to minimize the following overall loss function during the CART training:
\begin{equation}
   \mathcal{L}= {1\over{|D_l|}}{\sum_{y_j \in D_l}{(y_j - \overline{y}_{D_l})}^2} + {1\over{|D_r|}}{\sum_{y_j \in D_r}{(y_j - \overline{y}_{D_r})}^2}
    \label{eq:loss}
\end{equation}
where $D_l$ and $D_r$ denote the left and right division from a split, respectively. This ensures that the divisions would contain data samples with similar performance values (\textbf{Property 1}) while they are formed with respect to the similar values of the key configuration options as determined by the splits/thresholds at the finest granularity (\textbf{Property 2}), i.e., the more important options would appear on the higher level of the tree with excessive splitting.

However, here we do not use CART to generalize prediction directly on new data once it is trained as it has been shown that the splits and simple average of performance values in the division alone can still fail to handle the complex interactions between the options, leading to insufficient accuracy~\cite{DBLP:conf/icse/HaZ19}. Further, with our loss function in Equation~\ref{eq:loss}, CART is prone to be overfitting, especially for software quality data~\cite{DBLP:journals/ese/KhoshgoftaarA01}. This exacerbates the issue of sample sparsity~\cite{DBLP:journals/corr/abs-2202-03354} under a small amount of data samples which is not uncommon for configurable software systems~\cite{DBLP:conf/icse/HaZ19,DBLP:conf/esem/ShuS0X20}. 

% two reasons for not using the average in CART: 1, overfitting caused by not considering interaction; 2, there may still be non-split point features invovled in a division, which cause feature sparsity issue.
% the above obscure the benifit that could have been brounght by handling sample sparsity from the divisions.

Instead, what we are interested in are the (branch and/or leaf) divisions generated therein (with respect to the training data), which enable us to use further dedicated and more focused local models for better generalizing to the new data (lines 6-11 in Algorithm~\ref{alg:dal-code}). As such, the final prediction is no longer a simple average while we do not care about the CART overfitting itself as long as it fits the training data well. This is similar to the case of unsupervised clustering for which the clustering is guided by implicit labels (via the loss function at Equation~\ref{eq:loss}). Specifically, in \Model~we extract the data samples according to the divisions made by the $d$th depth of the CART, including all the leaf divisions with depth smaller than $d$. An example can be seen from Figure~\ref{fig:DT_example}, where $d$ is a controllable parameter. In this way, \Model~divides the data into a range of $[d+1,2^{d}]$ divisions ($d \geq 0$), each of which will be captured by a local model learned thereafter\footnote{When $d=0$, \Model~is basically equivalent to a single local model.}. Note that when the number of data samples in the division is less than the minimum amount required by a model, we merge the two divisions of the same parent node.


%Now, we train a DT regressor using all the weighted training samples, such that the DT can capture the influence and interactions between all the features and the performance. We choose DT because it has been commonly accepted as a good method to handle the influence of features and partition the training data into subsets, with explainable and visualizable decision makings~\cite{DBLP:conf/kbse/SarkarGSAC15,DBLP:journals/ese/GuoYSASVCWY18,DBLP:journals/ase/NairMSA18,DBLP:conf/icse/Chen19b,DBLP:journals/tse/ChenB17,DBLP:journals/corr/abs-1801-02175,DBLP:conf/kbse/GuoCASW13}.

%Next, we extract the branching conditions of DT (a set of $m$ splitting nodes $\overline{n}=(n_{1}, n_{2}, \cdots, n_{m})$ and a set of $m$ splitting thresholds $\overline{t}=(t_{1}, t_{2}, \cdots, t_{m})$) and use them as the guides for splitting the training samples. Because DT regressor finds the best branching features by minimizing squared error, it ensures that at every tree node, the samples are split in the best way that ML models can learn. Particularly, at every depth $d$, the DT splits the samples into at most $2^{d}$ nodes, and we follow this number of nodes to divide the training samples, i.e., the \Model~framework divides data into at most $2^{d}$ subsets, where $d$ is a hyperparameter decided by the user. Note that when the number of samples in the subset is less than the least amount needed by the learning model, we merge the two subsets of the same parent node.

As a concrete example, from Figure~\ref{fig:DT_example}, we see that there are two depths: when $d=1$ there would be two divisions (one branch and one leaf) with 10 and 8 samples respectively; similarly, when $d=2$ there would be three leaf divisions: two of each have 5 samples and one is the division with 8 samples from $d=1$ as it is a leaf. In this case, CART has detected that the \texttt{rtQuality} is a more important (binary) option to impact the performance, and hence it should be considered at a higher level in the tree. Note that for numeric options, e.g., \texttt{threads}, the threshold of splitting (\texttt{threads} $>5$) is also tuned as part of the training process of CART.

Indeed, since $d$ is such a critical parameter for \Model, setting the right value for it can be time-consuming and error-prone. In what follows, we will delineate the adaptive mechanism in \Model~that allows dynamic adaptation of the $d$ value during training. 

%where there two levels of nodes and samples are divided twice and resulting in four subsets. In the first depth, there are 84 samples, and DT split them based on the feature1 with threshold 0.5, i.e., samples whose feature1 is less or equal to 0.5 is split into the left cluster and vise versa. From the Figure we can see that feature1 is a binary feature, because there are only samples at $feature1=0$ and $feature1=1$. Besides, the dotted lines in the figure denote the mean values of the samples in the subsets, therefore it is clear the 45 samples in the left subset has a significant lower mean value, while the mean performance of the other set is hundreds of times higher. In depth2, the subsets are partitioned again via feature6 and 9, respectively, and we can see they are numerical features.


\subsubsection{Adapting the Depth $d$}


Since more divisions mean that the sample space is separated into more loosely related regions for dealing with the sample sparsity, one may expect that the accuracy will be improved, or at least, stay similar, thereby we should use the maximum possible $d$ from CART in the \textit{Dividing} phase. This, however, only exists in the ``utopia case'' where there is an infinite set of configuration data samples.

In essence, with the design of \Model, the depth $d$ will manage two conflicting objectives that influence its accuracy:

\begin{enumerate}
    \item greater ability to handle sample sparsity by separating the distant samples into divisions, each of which is learned by an isolated local model;
    \item and a larger amount of data samples in each division for the local model to be able to generalize.
\end{enumerate}

Clearly, a greater $d$ may benefit the ability to handle sample sparsity but it will inevitably reduce the data size per division for a local model to generalize since it is possible for CART to generate divisions with imbalanced sample sizes. From this perspective, we see $d$ as a value that controls the trade-off between the two objectives, and neither a too small nor too large $d$ would be ideal, as the former would lose the ability to deal with sample sparsity while the latter would leave too little data for a local model to learn, hence produce negative noises to the overall prediction. As a result, setting $d$ for a given system is crucial when using \Model. 

However, finding the appropriate $d$ value is not straightforward, as it often requires repeatedly profiling different values following in a trial-and-error manner, which can be rather expensive, especially when the best $d$ varies depending on the system (see Section []). To overcome this, in \Model, we design an adaptive mechanism as part of the \textit{Dividing} phase that is able to dynamically find the $d$ such that those two objectives can be balanced.

Specifically, we use the following functions to measure the ability to handle sample sparsity and the amount of information for a division $D_i$:
\begin{equation}
\begin{cases}
z_1(D_i)={1\over{|D_i|}}{\sum_{y_j \in D_i}{(y_j - \overline{y}_{D_i})}^2}\\
z_2(D_i)=n_i\\
\end{cases}
\label{eq:adapt}
\end{equation}
whereby $n_i$ is the number of samples assigned. $z_1$ is basically the mean square error (or performance variance of the samples in a division) taken from the loss function (Equation~\ref{eq:loss}) that splits the divisions with respect to the important configuration options. As such, the samples in a division that is generally closer to each other in terms of the performance value, after being divided according to the importance of key configuration options, are more likely to be beneficial for a local model to learn. Intuitively, $z_1$ is to be minimized while $z_2$ needs to be maximized. Given a CART that generates a maximum number of $d_{max}$ divisions under the given training data, our purpose is to find the $d$ value ($0\leq d\leq d_{max}$) that leads to the highest number of ``knee divisions'' (a.k.a knee points []) in the objective space of $z_1$ and $z_2$ for the divisions generated by all possible $d$ values. In essence, from a multi-objective optimization perspective, knee points represent the solutions that, when changed, can only marginally improve one objective by largely comprising the other [], hence achieving a well-balanced trade-off.

\input{Tables/alg2}

Algorithm~\ref{alg:adapt-code} illustrates the proposed adaptive mechanism with the following key steps:

\begin{enumerate}%[Step 1:]
    \item For each division and its corresponding $d$ value, i.e., a vector $<D_i,d_j>$, calculating the objective value of $z_1$ and $z_2$ for $D_i$.
    \item Retain the non-dominated divisions with respect to $z_1$ and $z_2$ while discarding the others.
    \item Find the ``knee divisions'' in the objective space of $z_1$ and $z_2$ using the following equation:
\begin{equation}
pd(D_i, \ell)=
\left\{
  \begin{array}{lr}	
    \frac{|\epsilon|}{\sqrt{a^2+b^2}}, & {if}\quad \epsilon < 0\\
    -\frac{|\epsilon|}{\sqrt{a^2+b^2}}, & {otherwise}\\
  \end{array}
\right.
\label{eq:knee}
\end{equation}
    where $pd(D_i, \ell)$ is the perpendicular distance from each non-dominated division to the line $\ell$ formed by the extreme divisions with the best value of $z_1$ and $z_2$, respectively; $\epsilon$ is the mathematical function of $\ell$, which is $\epsilon=a\times f(\mathbf{x})+b\times g(\mathbf{x})+c$, and the coefficients can be easily calculated using the extreme divisions $D_{z_1}$ and $D_{z_2}$. $\epsilon<0$ means that $D_i$ is on the left side of $\ell$; otherwise, $D_i$ is on the right side of $\ell$. Clearly, divisions on the left side of $\ell$ are preferable to those on the right when we convert both objectives as minimizing ones. Therefore, the division(s) with the largest $pd(D_i, \ell)$ value would be the knee, and the corresponding vectors $<D_i,d_j>$ are put into a set $\mathbfcal{C}$.
    
    \item Count the number of divisions that are considered as the knee for each of the $d_j$ from $\mathbfcal{C}$, the $d$ value with the highest count would be chosen for our \Model.
\end{enumerate}

Apart from the above main procedure, there are also a few special cases that we need to handle in an alternative way:

\begin{itemize}
    \item In \textit{step 2}, if there is only one non-dominated division then clearly the corresponding $d$ value would be chosen.
    \item In \textit{step 2}, if there are only two non-dominated divisions then the smaller $d$ would be used since no other points for calculating the perpendicular distance.
    \item In \textit{step 4}, if multiple $d$ values have the same highest count, we use the smaller $d$ to avoid training unnecessary local models.
\end{itemize}

With such an adaptive mechanism of $d$, we strike a balance for the aforementioned objectives while requiring neither additional training nor profiling. The computational overhead of finding the knee division(s) is also ignorable, as we will show in Section [].

%Similar to the fact that we cannot theoretically justify how much data is sufficient for a model to learn the concept~\cite{DBLP:conf/dyspan/OyedareP19}, it is also difficult to prove how many divisions are sufficient for handling the sample sparsity in performance modeling. However, in Section~\ref{subsec:rq3}, we will empirically demonstrate that there is a (upward) quadratic correlation between $d$ value and the error incurred by \Model~due to the conflict between the above two goals. 


\subsection{Training}


Given the divisions generated by the \textit{Dividing} phase, we train a local model for the samples from each division identified as part of \textbf{Goal 2} (lines 12-14 in Algorithm~\ref{alg:dal-code}). 
\textcolor{red}{Theoretically, we can pair them with any model given the generic concept of divisible learning. However, we adopt the state-of-the-art regularized Hierarchical Interaction Neural Network~\cite{DBLP:journals/tosem/ChengGZ23} (namely HINNPerf) as we provide compelling empirical evidence on its effectiveness under \Model~when handling feature sparsity and the interaction therein well for configurable software, even with small training sample size. Section~\ref{subsec:local} reports on our use and observation of~\cite{DBLP:journals/tosem/ChengGZ23}}
% Theoretically, we can pair them with any model given the generic concept of divisible learning. However, as we will show in Section~\ref{subsec:rq2}, the state-of-the-art regularized hierarchical interaction Neural Network~\cite{DBLP:journals/tosem/ChengGZ23} (namely \texttt{HINNPerf}), published at TOSEM'23, is the most effective one under \Model~as it handles feature sparsity and the interaction therein well for configurable software. Indeed, Cheng \textit{et al.}~\cite{DBLP:journals/tosem/ChengGZ23} showed that \texttt{HINNPerf} is more effective than the others even with small data samples when predicting software configuration performance (in our study, we also evaluate the same systems with small training sample sizes as used in their work). Therefore, in \Model~we choose \texttt{HINNPerf} as the underlying local model by default. 

%the state-of-the-art regularized Deep Neural Network (rDNN)~\cite{DBLP:conf/icse/HaZ19} (namely \texttt{DeepPerf}), published at ICSE'19, is the most effective one under \Model~as it handles feature sparsity well for configurable software. Indeed, Ha and Zhang~\cite{DBLP:conf/icse/HaZ19} showed that rDNN is more effective than the others even with small data samples when predicting software performance (in our study, we also evaluate the same systems with small training sample sizes as used in their work). Therefore, in \Model~we choose rDNN as the underlying local model by default. 

In this work, we adopt exactly the same structure and training procedure as those used by Cheng \textit{et al.}~\cite{DBLP:journals/tosem/ChengGZ23}, hence we kindly refer interested readers to their work for the training details~\cite{DBLP:journals/tosem/ChengGZ23}. Since the local models of the divisions are independent, we utilize parallel training as part of \Model. 

It is worth noting that, as we will show in Section [], \Model~is capable of improving a wide range of local models compared with the case when they are used to learn the entire configuration data space.

%In this work, we adopt exactly the same structure and training procedure as those used by Ha and Zhang~\cite{DBLP:conf/icse/HaZ19}, hence we kindly refer interested readers to their work for the training details~\cite{DBLP:conf/icse/HaZ19}. Since the local models of the divisions are independent, we utilize parallel training as part of \Model. 
 
 %including:
% \textcolor{red}{
% (1) Scaling/normalization is applied to the data; (2) The number of neurons on the input layer is equal to the number of configuration options; (3) $L_{1}$ regularization is applied to the first hidden layer to prevent overfitting; (4) The number of neurons on each hidden layer is 128; (5) The ReLU activation function is used for each hidden layer; (6) The training epoch is set to 2000; (7) Adam optimizer is used to find the optimal number of hidden layers, learning rate, \textit{etc}.
% }

% \begin{itemize}
%     \item Scaling/normalization is applied to the data. % they scale both configuration and performance
%     \item The number of neurons on the input layer is equal to the number of configuration options.
%     \item $L_{1}$ regularization is applied to the first hidden layer to prevent overfitting.
%     \item The number of neurons on each hidden layer is 128.
%     \item The ReLU activation function is used for each hidden layer.
%     \item The training epoch is set to 2000.
%     \item Adam optimizer is used to find the optimal number of hidden layers, learning rate, \textit{etc}.
% \end{itemize}




% We use this architecture because it has been proven to produce state-of-the-art results for performance learning tasks. Then, the training process is also the same as~\cite{DBLP:conf/icse/HaZ19}, in detail:
% \begin{itemize}
%     \item The loss function is the mean square error of the predicted performance and the actual performance.
%     \item The features are scaled between 0 and 1, while the labels are scaled to 0-100.
%     \item Adam optimizer is adopted to train the DNN
% \end{itemize}

%\input{Tables/alg3}

\subsection{Predicting}

When a new configuration arrives for prediction, \Model~chooses a local model of division trained previously to infer its performance. Therefore, the question is: how to assign the new configuration to the right model (\textbf{Goal 3})? A naive solution is to directly feed the configuration into the CART from the \textit{Dividing} phase and check which divisions it associates with. Yet, since the performance of the new configuration is unforeseen from the CART's training data, this solution requires CART to generalize accurately, which, as mentioned, can easily lead to poor results because CART is overfitting-prone when directly working on new data~\cite{DBLP:journals/ese/KhoshgoftaarA01}.


%given that the divisions from the \textit{Dividing} phase in fact serve as the pseudo labels on what kinds of configurations should be clustered together,

Instead, by using the divided samples from the \textit{Dividing} phase (which serves as pseudo labeled data), we train a Random Forest---a widely used classifier and is resilient to overfitting ~\cite{DBLP:conf/splc/ValovGC15,DBLP:conf/oopsla/QueirozBC16,DBLP:conf/icse/0003XC021}---to generalize the decision boundary and predict which division that the new configuration should be better assigned to (lines 15-21 in Algorithm~\ref{alg:dal-code}). Again, in this way, we are less concerned about the overfitting issue of CART as long as it matches the patterns of training data well. This now becomes a typical classification problem but there are only pseudo labels to be used in the training. Using the example from Figure~\ref{fig:DT_example} again, if $d=1$ is chosen as the best value then the configurations in the 10 sample set would have a label \textit{``division1''}; similarly, those in the 8 sample set would result in a label \textit{``division2''}.


However, one issue we experienced is that, even with $d=1$, the sample size of the two divisions can be rather imbalanced, which severely harms the quality of the classifier trained. For example, when training \textsc{BDB-C} with 18 samples, the first split in CART can lead to two divisions with 14 and 4 samples, respectively.
% \textcolor{red}{please give a concrete example.} 
Therefore, before training the classifier we use Synthetic Minority Oversampling Technique (SMOTE)~\cite{DBLP:journals/bmcbi/BlagusL13a} to pre-process the pseudo label data, hence the division(s) with much fewer data (minority) can be more repeatedly sampled.

%which further consolidates the generalizability.

Finally, the classifier predicts a division whose local model would infer the performance of the new configuration.




%Finally, the local model, which is trained on the division predicted by the classifier, would infer the performance of the new configuration (line 22 in Algorithm~\ref{alg:dal-code}).


==> tsne.tex <==
\begin{subfigure}{.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/Apache_AllNumeric_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{Apache}}
  \label{fig:TNSE-Apache}
\end{subfigure}
% ~\hfill
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/BDBC_AllNumeric_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{BDB-C}}
  \label{fig:TNSE-BDBC}
\end{subfigure}
% ~\hfill
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/BDBJ_AllNumeric_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{BDB-J}}
  \label{fig:TNSE-BDBJ}
\end{subfigure}


\begin{subfigure}{.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/kanzi_TSNE_scatter.pdf}  
  \vspace{-1cm} \caption{\textsc{kanzi}}
  \label{fig:TNSE-kanzi}
\end{subfigure}
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/sqlite_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{SQLite}}
  \label{fig:TNSE-SQLite}
\end{subfigure}
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/x264_AllNumeric_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{x264}}
  \label{fig:TNSE-x264}
\end{subfigure}


\begin{subfigure}{.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/Dune_AllNumeric_TSNE_scatter.pdf}  
  \vspace{-1cm} \caption{\textsc{Dune MGS}}
  \label{fig:TNSE-Dune}
\end{subfigure}
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/hipacc_AllNumeric_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{HIPA$^{cc}$}}
  \label{fig:TNSE-HIPAcc}
\end{subfigure}
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/hsmgp_AllNumeric_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{HSMGP}}
  \label{fig:TNSE-HSMGP}
\end{subfigure}


\begin{subfigure}{.33\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/Lrzip_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{Lrzip}}
  \label{fig:TNSE-Lrzip}
\end{subfigure}
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/nginx_TSNE_scatter.pdf} 
  \vspace{-1cm} \caption{\textsc{nginx}}
  \label{fig:TNSE-nginx}
\end{subfigure}
\hspace{-0.2cm}
\begin{subfigure}{.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/VP8_TSNE_scatter.pdf}  
  \vspace{-1cm} \caption{\textsc{VP8}}
  \label{fig:TNSE-VP8}
\end{subfigure}

